Persuasion in Networks: Can the Sender Do Better than Using Public Signals?

Political and advertising campaigns increasingly exploit social networks to spread information and persuade people. This paper studies a persuasion model to examine whether such a strategy is better than simply sending public signals. Receivers in the model have heterogeneous priors and will pass on a signal if they are persuaded by it to take sender's preferred action. I show that a risk-neutral or risk-loving sender prefers to use public signals, unless the more sceptical receivers are sufficiently more connected in the network. This result still holds when the network exhibits homophily. When the sender is risk averse or has a threshold function as payoff function, I characterise conditions under which the sender prefers to exploit the network. An important factor identified by these conditions is whether the less sceptical receivers are sufficiently connected.

==> online_app_reserve.tex <==


\section{Appendix for Online Publication}
	\subsection{Formal Definition of Branching Process}
		To formally define the branching processes, I first define two sets of random variables. 
	Let $\mathcal{N}$ denote the set of all vectors whose entries are positive integers, i.e. $\mathcal{N} \equiv \cup_{x \in \mathbb{N}} (\mathbb{N} \cup 0)^{x}$ where $\mathbb{N}$ is the set of natural numbers. There are two sets of vector valued random variables, $\{X^{h}_{i}\}_{i \in \mathcal{N} }$ and $\{X^{l}_{i}\}_{i \in \mathcal{N}  }$. All these random variables are mutually independent. $X^{t}_{i} = (X^{t}_{i,h}, X^{t}_{i,l} )$ are identically distributed in the following way: distribution of $\tilde{d} = X^{t}_{i,h}+ X^{t}_{i,l}$ is $\tilde{p}_{\tilde{d}}^{t}$. Conditional on $\tilde{d}$, $X^{t}_{i,h}$ is distributed according to binomial distribution with $\tilde{d}$ trials and success probability $q_{t}$. 
	
	For $t \in \{h,l\}$, the branching process
	$\tilde{ \mathcal{B}}(D|h)$  is a random tree formed in the following way
	\begin{enumerate}
		\item The branching process is a sequence of random variables $\{S_{n}\}_{n \in \mathbb{N}}$. $S_{1}$ contains node 1 with type $h$. 
		\item For all $i \in \mathcal{N}$, if $i$ is in generation $n$, it generates period $n+1$ offsprings according to $X^{t}_{i}$, i.e. $i$ generates $X^{t}_{i,h}$ type $h$ offsprings and $X^{t}_{i,l}$ type $l$ offsprings. These offsprings will have indices $\{(i,1),(i,2),...(i+\tilde{d}) \}$, where $\tilde{d} = X^{t}_{i,h}+ X^{t}_{i,l}$. $(i,x)$ is the vector formed by appending $x$ to the vector $i$. 
		\item More formally, let $t_{i}$ denote type of node $i$. We have $S_{1}=\{(1,t_{1})\}$ and $t_{1}=h$.
		\item For each $i \in \mathcal{N}$ and type $t \in \{h,l\}$, define a random variable \[S^{i}_{t} \equiv \{((i,1),t(i,1)),...((i,\tilde{d}),t(i,\tilde{d}))\}\] where $\tilde{d} = X^{t}_{i,h}+ X^{t}_{i,l}$ and \[
		t(i,x) = \begin{cases}
			h & \text{if } 1 \le x \le X^{t}_{i,h} \\
			l & \text{if } X^{t}_{i,h}+1 \le x \le \tilde{d}
		\end{cases}
		\]
		\item Given $S_{n}$, $S_{n+1}$ is the random variable
		\[
		S_{n+1} = \cup_{(i,t_{i}) \in S_{n}} S^{i}_{t_{i}}
		\]
	\end{enumerate}
	Note that a node in the branching process is a pair of index and type, but by how the process is defined, there can't be two nodes with the same index. Therefore, when the type of node is not important, I omit it and just refer to a node by its index. For example, a typical node will be node $i$ rather than node $(i,t)$. Similarly, I use $i \in S_{n}$ to represent that either $(i,h)$ or $(i,l)$ is in $S_{n}$. 
	
	$\tilde{ \mathcal{B}}(D|l)$ differs from $\tilde{ \mathcal{B}}^{h}(D)$ only in the type of node in the first generation $S_{1}$. For $\tilde{ \mathcal{B}}(D|l)$, we have $t_{1}=l$ instead of $t_{1}=h$. Given $S_{n}$, $S_{n+1}$ is produced in the same way. 
	
	The branching process $\mathcal{B}(D)$ is defined as follows,
	\begin{enumerate}
		\item $S_{0}$ again contains node 1. $t_{1}$ is equal to $h$ with probability $\gamma_{h}$ and $l$ with probability $\gamma_{l}$. 
		\item Given $t_{1}$, it produces offspings according to $p_{d}^{t_{1}}$. Given its number of offsprings $d$, the distribution over its number of type $h$ offsprings is binomial distribution with $d$ trials and success probability $q_{t_{1}}$.  
		\item For $n \ge 1$, given $S_{n}$, $S_{n+1}$ is produced in the same way as $\tilde{ \mathcal{B}}^{h}(D)$. Again, all nodes produce offsprings mutually independently of each other. 
	\end{enumerate}
	Recall that $\rho_{D}(m)$ and $\tilde{\rho}_{D}(m|t)$ denote the probability that the branching process contains less than $m$ nodes for $\mathcal{B}(D)$ and $\tilde{ \mathcal{B}}(D|t)$ respectively. Also, $\rho_{D}^{h}(m)$ and $\tilde{\rho}^{h}_{D}(m|t)$ respectively denote the probability $\mathcal{B}(D)$ and $\tilde{ \mathcal{B}}(D|t)$ contain less than $m$ nodes after deleting nodes with type $l$ ancestors except root node. I use $S_{n}^{h}$ to denote nodes left in generation $n$ after deleting all nodes with type $l$ ancestors except the root node.
	
	We can now write $\rho_{D}(\infty) \equiv1- \lim_{n \rightarrow \infty}Pr_{\mathcal{B}(D)}(|S_{n}|=0  ) $, and similarly for $\tilde{\rho}_{D}(\infty|t)$. Again, we need to study networks after deleting all type $l$ nodes and we can write $\rho_{D}^{h}(\infty) \equiv1- \lim_{n \rightarrow \infty}Pr_{\mathcal{B}(D)}(|S_{n}^{h}|=0  ) $, and similarly for $\tilde{\rho}^{h}_{D}(\infty|t)$.
	The following remark says that a branching process contains infinitely many nodes if and only if it doesn't go extinct. 
	\begin{remark}
		For all three branching processes defined above and any $n$, $Pr(\sum_{n} |S_{n}| > M)$ converges to 0 as $M$ goes to infinity.  
	\end{remark}
	\begin{proof}
		By first part of lemma 4 in \citet{sadler2020}, for any $\epsilon>0$, we can find a $d$ large enough that the probability all nodes within generation $n$ has less than $d$ offsprings at least $1-\epsilon$. If all nodes within generation $n$ produces less than $d$ nodes, then there are at most $1 + d^{n}$ nodes within generation $n$. 
		Since $\epsilon$ is arbitrary, the result follows. 
	\end{proof}
	It's trivial that $1 - Pr_{\mathcal{B}(D)}(|S_{m+1}|=0  )   \le 1- \rho_{D}(m)$. The remark above implies that $ Pr_{\mathcal{B}(D)}(|S_{m}|=0  ) \le \lim_{M \rightarrow \infty} \rho_{D}(M)$ for all $m$. Combining these, we get $\rho_{D}(\infty) = 1- \lim_{m \rightarrow \infty}\rho_{D}(m)$.
	The same reasoning shows that $\tilde{\rho}_{D}(\infty|t) = 1- \lim_{m \rightarrow \infty}\tilde{\rho}_{D}(m|t)$ for $t \in \{h,l\}$, and the same results for $\rho_{D}^{h}(\infty)$ and $\tilde{\rho}_{D}^{h}(\infty|t)$. This proves remark \ref{remark2}. 
	
	I now provide the formal argument for remark \ref{remark3} reproduced below \\
	\textbf{Remark 3.}
	\textit{	For all three branching processes defined above, conditional on there being $d_{h}$ type $h$ nodes and $d_{l}$ type $l$ nodes in second generation, the probability that the process never dies out is}
		\[
		1-(1-\tilde{\rho}_{D}(\infty|l))^{d_{l}}(1-\tilde{\rho}_{D}(\infty|h))^{d_{h}}
		\]
		\textit{Also, conditional on there being $d_{h}$ type $h$ nodes and $d_{l}$ type $l$ nodes in second generation, the probability that they never die out after deleting nodes with type $l$ ancestors except root node is given by}
		\[
		1- ( 1 - \tilde{\rho}^{h}_{D}(\infty|h)   )^{d_{h}}
		\]
	\begin{proof}
		In short, from construction of these processes, the part of a process that has some second generation node of type $t$ as its ancestor behaves in exactly the same way as $\tilde{\mathcal{B}}(D|t)$. This is because this second generation node of type $t$ produces offsprings in exactly the same way as the initial node in $\tilde{\mathcal{B}}(D|t)$, and all their future generation offsprings also produce offsprings in the same way. Also, all nodes produce offsprings independently of each other. Therefore, if there are $d_{h}$ type $h$ nodes and $d_{l}$ type $l$ nodes in the second generation, the process behaves in the same way as having $d_{h}$ independent processes that behave as $\tilde{\mathcal{B}}(D|h)$ and $d_{l}$ independent processes that behave as $\tilde{\mathcal{B}}(D|l)$. I now give a more detailed argument.
		
		For each node with index $i$ in generation 2, we can define a sequence of random variables
		$\{S_{n,i}\}_{n \ge 2}$ where $S_{n,i} \equiv \{(j,t) | (j,t) \in S_{n}, j=(i,x) \text{where }x \in \mathbb{N}^{n-2}\}$. Intuitively, $\{S_{n,i}\}_{n \ge 2}$ is the subtree or sub branch that is produced by node $i$. 
		
		We know that $|S_{n}|=0$ iff $|S_{n,i}|=0$ for all $i \in S_{2}$. By construction of all these branching processes, $S_{n,i}$ is determined by random variables $X_{j}^{t}$ where $j=(i,x)$ for some vector $x \in \mathcal{N}$. Since all these $X_{j}^{t}$ are mutually independent, the random variables $\{|S_{n,i}|\}_{i \in S_{2}}$ are mutually independent. 
		
		We know that type $h$ and type $l$ nodes in any $S_{n,i}$ produce offsprings in the same way as type $h$ and type $l$ nodes in $\tilde{\mathcal{B}}(D|l)$ or $\tilde{\mathcal{B}}(D|l)$. Therefore, the following two random variables have the same distribution
		\begin{enumerate}
			\item the number and type of nodes in $S_{n+1,i}$ conditional on $d_{h}'$ type $h$ nodes and $d_{l'}$ type $l$ nodes in $S_{n,i}$.
			\item For $\tilde{\mathcal{B}}(D|h)$ and $\tilde{\mathcal{B}}(D|l)$, the number and type of nodes in $S_{n}$ conditional on $d_{h}'$ type $h$ nodes and $d_{l'}$ type $l$ nodes in $S_{n-1}$.
		\end{enumerate}
		If node $i \in S_{2}$ is type $t$, then trivially $S_{2,i}$ and $S_{1}$ for $\tilde{\mathcal{B}}(D|t)$ contain the same number of type $h$ and type $l$ nodes. Applying the observation above repeatedly implies that if $i$ has type $t$, then $\lim_{n \rightarrow \infty} Pr(|S_{n,i}|=0) = \tilde{\rho}_{D}(\infty|t)$. The claim then follows from independence. 
		
		The argument above goes through by replacing all $S_{n}$ with $S_{n}^{h}$, $S_{n,i}$ with $S_{n,i}^{h}$ and $\tilde{\rho}_{D}(\infty|t)$ with $\tilde{\rho}_{D}^{h}(\infty|t)$. Recall that quantities with superscript $h$ are counterparts of those without $h$ in the processes obtained by deleting all nodes with type $l$ ancestors. 
	\end{proof}

	\subsection{Proof for Voting Game}
	I first study the optimal public signals for the sender. If a signal doesn't convince type $l$ receivers, then sender gets payoff 0 when that signal is realised and visible. 
	If a signal convinces type $l$ receivers, then it must convince everyone and sender gets payoff 1 when that signals is realised and visible. Therefore, sender's optimal strategy must maximise the probability that type $l$ receivers are convinced. This is precisely the hard news strategy. Therefore, sender's optimal payoff using public signals (in the limit as $n \rightarrow \infty$) is 
	\[
	V_{hard} = \mu_{s}(\omega=1) + \mu_{s}(\omega=0)\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=1)}
	\]  
	
	To analyse network signals, I introduce the following definition. Define $d_{vote}$ to be the smallest $d$ such that
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} \frac{ 1 - \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1) }\hat{\zeta}(l,d) }{1 - \hat{\zeta}(l,d) } \ge 1
	\]
	Let $d_{vote}$ be $\infty$ if there exists no such $d$. As shown in proof of the next proposition, if a type $l$ receiver has degree lower than $d_{vote}$, then she can't choose action 1 upon observing $\emptyset$. Using this definition, we can provide a necessary condition and a sufficient condition for network signals to outperform public signals. Intuition for why $d_{vote}$ is important is provided after statement of the proposition. 
		\begin{proposition} \label{propvotinggame}
		A necessary condition for $V_{net}^{*} > V_{hard}$ is
		\[
		\sum_{d \ge d_{vote}} \gamma_{l}p_{d}^{l} \ge \overline{x} - \gamma_{h}
		\]
		A sufficient condition is
		\[
		\sum_{d \ge d_{vote}+1} \gamma_{l}p_{d}^{l}(1-\hat{\zeta}(l,d)) > \overline{x} - \gamma_{h}
		\]
	\end{proposition}
	
	\textit{Proof of Proposition \ref{propvotinggame} :}\\
	By lemma \ref{lemmaprobongiant2}, it must be the case that $\hat{\zeta}(l,d)=0$ for all $d$, or $\hat{\zeta}(l,d)>0$ for all $d$. Also, if it's not the case that $\hat{\zeta}(l,d)=0$ for all $d$, then $\hat{\zeta}(l,d)$ converges to 1 as $d$ converges to infinity. This implies that as long as $\frac{\hat{L}_{1}}{n}$ doesn't converge in probability to 0, then $d_{vote}$ is finite. 
	One can verify that when $d_{vote}$ is finite, the ratio
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{1-  \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)}   \hat{ \zeta }(l,d)  }{1-   \hat{ \zeta }(l,d) } 
	\]
	is weakly larger than 1 iff $d \ge d_{vote}$. By definition, the ratio is smaller than 1 for all $d$ if $d_{vote}$ is $\infty$.
	
	I show the necessary condition first. Suppose that the necessary condition stated in proposition doesn't hold, i.e. $\gamma_{h} + \sum_{d > d_{vote}}\gamma_{l}p_{d}^{l} < \overline{x}$. 
	By definition of $d_{vote}$ and hypothesis, we can find a $\beta>0$ small enough such that 
	\begin{enumerate}
		\item \[
		\hat{ \zeta }(l,d) +3 \beta <1	 \quad \text{ and } \quad  \frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{1-  \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)} (2\beta+  \hat{ \zeta }(l,d) ) }{1-   \hat{ \zeta }(l,d) - 3\beta} < 1
		\]
		for all $d < d_{vote}$.
		\item $\gamma_{h}+ \beta + \sum_{d > d_{vote}}\gamma_{l}p_{d}^{l} < \overline{x}$.
	\end{enumerate}
	
	We know that the proportion of type $h$ receivers converge to $\gamma_{h}$, and $\sum_{d \ge d_{vote}}\frac{N_{t,d}}{n}$ converges to $\sum_{d \ge d_{vote}} \gamma_{l}p_{d}^{l}$. Therefore, for fixed $\beta$ satisfying conditions above, we can find some $n_{1}$ such that for all $n>n_{1}$, 
	\begin{enumerate}
		\item $Pr(g^{n} \in \mathcal{A}(\beta,\overline{d})) \ge 1- \beta$
		\item $ \frac{N_{h}}{n} + \sum_{d \ge d_{vote}} \frac{N_{t,d}}{n} \in [\gamma_{h}+ \sum_{d \ge d_{vote}}\gamma_{l}p_{d}^{t}-\beta,\gamma_{h}+ \sum_{d \ge d_{vote}}\gamma_{l}p_{d}^{t}+\beta ] $
	\end{enumerate} 
	
	Suppose that sender uses some strategy $\Pi^{n}$ in the game with $n \ge n_{1}$ receivers. Let $S_{good}$ denote the set of signals that convince both types of receivers, $S_{int}$ denote the set of signals that convince only type $h$ receivers and $S_{bad}$ as those that convince neither. 
	Let $OB_{good}(d,\omega;\Pi^{n}) $ denote the probability that a type $l$ receiver with degree $d$ observe observe signals in $S_{good}$ under $\Pi^{n}$. Similarly let $OB_{int}(d,\omega;\Pi^{n}) $ denote the probability that a type $l$ receiver with degree $d$ observe observe signals in $S_{int}$ under $\Pi^{n}$. We know that the probability of observing signals in $S_{bad}$ is smaller than $\beta$. As in other proofs, let $\alpha(\emptyset,l,d;\Pi^{n})$ denote type $l$ receivers action upon observing $\emptyset$.
	
	I first show $\alpha(\emptyset,l,d;\Pi^{n})=0$ for all $d < d_{vote}$ by contradiction. Suppose that $\alpha(\emptyset,l,d;\Pi^{n})=1$ for some $d < d_{vote}$. The likelihood ratio for type $l$ receiver with degree $d$ upon observing $\emptyset$ must be weakly greater than 1, i.e.
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{1- OB_{good}(d,\omega=1;\Pi^{n})-OB_{int}(d,\omega=1;\Pi^{n}) }{1- OB_{good}(d,\omega=0;\Pi^{n})-OB_{int}(d,\omega=0;\Pi^{n})-\beta} \ge 1
	\]
	By lemma \ref{lemmanonemptysignalposterior}, we know that $\frac{OB_{good}(d,\omega=1;\Pi^{n})}{OB_{good}(d,\omega=0;\Pi^{n})} \ge \frac{\mu_{l}(\omega=0)}{\mu_{l}(\omega=1)}$ and $\frac{OB_{int}(d,\omega=1;\Pi^{n})}{OB_{int}(d,\omega=0;\Pi^{n})} \ge \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)}$. Therefore, we must have 
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} \frac{1-   \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)}K }{1-  K -\beta} \ge 1
	\]
	for any $ K \in [OB_{int}(d,\omega=0;\Pi^{n}), 1-\beta) $.
	
	$OB_{int}(d,\omega=0;\Pi^{n})$ is $\pi(s|\omega=0)$ times the probability of observing $s$ conditional on it being realised. By properties of $\mathcal{A}(\beta,\overline{d})$ and our choice of $n$, the probability of observing $s$ conditional on it being realised is at most $2\beta + \hat{\zeta}(l,d)$.
	By how $\beta$ is chosen, we have $2\beta + \hat{\zeta}(l,d) < 1-\beta$, which in turn implies 
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{1-  \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)} (2\beta+  \hat{ \zeta }(l,d) ) }{1-   \hat{ \zeta }(l,d) - 3\beta} \ge 1
	\]
	But this inequality is a contradiction with how $\beta$ is chosen, so $\alpha(\emptyset,l,d;\Pi^{n})=0$ for all $d < d_{vote}$.
	
	We can bound sender's payoff by assuming that when signals in $S_{int} \cup S_{bad}$ are realised or when signals are not visible, all type $h$ nodes choose action 1 and all type $l$ nodes use their optimal action upon observing $\emptyset$. Sender's payoff can thus be bounded above by
	\begin{equation} \label{voteeq1}
		\sum_{\omega}\mu_{s}(\omega) \big[b(\omega)\sum_{s \in S_{good}}\pi(s|\omega) + (1-b(\omega)\sum_{s \in S_{good}}\pi(s|\omega))v(\frac{N_{h}}{n} + \sum_{d}\alpha(\emptyset,l,d;\Pi^{n})\frac{N_{l,d}}{n})\big]
	\end{equation}
	Since $b(\omega=1)\sum_{s \in S_{good}}\pi(s|\omega=1) \le 1$ and $b(\omega=0)\sum_{s \in S_{good}}\pi(s|\omega=0) \le \frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}$, expression \ref{voteeq1} is weakly smaller than $V_{hard}$ if 
	\[
	\frac{N_{h}}{n} + \frac{\sum_{d}\alpha(\emptyset,l,d;\Pi^{n})N_{l,d}}{n} < \overline{x}
	\]
	Since $\alpha(\emptyset,l,d;\Pi^{n})=0 $ for all $d < d_{vote}$, we have
	\[
	\frac{N_{h}}{n} + \frac{\sum_{d}\alpha(\emptyset,l,d;\Pi^{n})N_{l,d}}{n} \le \frac{N_{h}}{n} + \frac{\sum_{d \ge d_{vote}} N_{l,d}}{n} < \gamma_{h} + \sum_{d \ge d_{vote}}\gamma_{l}p_{d}^{l} + \beta < \overline{x}
	\]
	This concludes proof for the necessary condition. 
	
	To show the sufficient condition, suppose that sender uses strategy $\Pi_{2}^{n}$ described as follows for all $n$,
	\[
	\pi_{2}(s|\omega=1)=\pi_{2}(s|\omega=0)=1 \qquad b_{2}(\omega=1)=\frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)} \qquad b_{2}(\omega=0) = 1
	\]
	Let the seeds always hit $\hat{L}_{1}$. One can verify that type $h$ receivers always choose action 1, regardless of what they observe. Let $OB_{s}(d,\omega;\Pi^{n}_{2})$ denote the probability that type $l$ receivers observes $s$ in state $\omega$ under strategy $\Pi_{2}^{n}$. Upon observing $\emptyset$, receivers with type $l$ and degree $d$ has likelihood ratio
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} \frac{1-OB_{s}(d,\omega=1;\Pi_{2}^{n}) }{1-OB_{s}(d,\omega=0;\Pi_{2}^{n})}
	\]
	$OB_{s}(d,\omega;\Pi^{n}_{2})$ is given by $b_{2}(\omega)E(\frac{N_{\hat{L}_{1},l,d}}{N_{l,d}})$. By lemma \ref{lemmaprobongiant}, $b_{2}(\omega)E(\frac{N_{\hat{L}_{1},l,d}}{N_{l,d}})$ converges to $b_{2}(\omega)\hat{ \zeta }(l,d)$, and thus the likelihood ratio converges to 
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} \frac{1- \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)}\hat{ \zeta }(l,d) }{1-\hat{ \zeta }(l,d)}
	\]
	If the sufficient condition holds, we can find some $\overline{d}'$ such that $\gamma_{h} + \sum_{d=d_{vote}+1}^{\overline{d}'} \gamma_{l}p_{d}^{l} (1-\hat{ \zeta }(l,d)) > \overline{x}$. By argument at the beginning of the proof, we can find $n_{2}$ large enough such that for all $n \ge n_{2}$, and $d_{min} < d \le \overline{d}'$, 
	\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} \frac{1-OB_{s}(d,\omega=1;\Pi_{2}^{n}) }{1-OB_{s}(d,\omega=0;\Pi_{2}^{n})} > 1
	\]
	Therefore, for $n \ge n_{2}$ sender's payoff is bounded below by
	\[
	\sum_{\omega}\mu_{s}(\omega)\big[ b_{2}(\omega)\sum_{g^{n}}Pr(g^{n}) v(\frac{N_{h}}{n} + \sum_{d=d_{vote}+1}^{\overline{d}'}\frac{N_{l,d}}{n}(1-\frac{N_{\hat{L}_{1},l,d}(g^{n})}{N_{l,d}})    ) +  (1-b(\omega))v( \frac{N_{h}}{n} + \sum_{d=d_{vote}+1}^{\overline{d}'}\frac{N_{l,d}}{n}   ) \big] 
	\]
	Since $\frac{N_{h}}{n}$ converges to $\gamma_{h}$, $\frac{N_{l,d}}{n}$ converges to $\gamma_{l}p_{d}^{l}$ and $\frac{N_{\hat{L}_{1},l,d}(g^{n})}{N_{l,d}}$ converges in probability to $\hat{ \zeta }(l,d)$, the expression
	\[
	\frac{N_{h}}{n} + \sum_{d=d_{vote}+1}^{\overline{d}'}\frac{N_{l,d}}{n}(1-\frac{N_{\hat{L}_{1},l,d}(g^{n})}{N_{l,d}})
	\]
	converges in probability to $\gamma_{h} + \sum_{d=d_{vote}+1}^{\overline{d}'} \gamma_{l}p_{d}^{l}(1-\hat{ \zeta }(l,d)) > \overline{x}$, which implies that 
	\[
	v(\frac{N_{h}}{n} + \sum_{d=d_{vote}+1}^{\overline{d}'}\frac{N_{l,d}}{n}(1-\frac{N_{\hat{L}_{1},l,d}(g^{n})}{N_{l,d}})    )
	\]
	converges in probability to $v(1)$. Therefore, the lower bound on sender's payoff above converges in probability to $v(1)$, which is strictly larger than $V_{hard} = \mu_{s}(\omega=1)v(1) + \mu_{s}(\omega=0)\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}v(1)$. This concludes the proof. 
	\qed
	

	\subsection{Proofs for extension in subsection 5.2}
	In this subsection, I allow the sender's seeding strategy to depend on the state. Also, I consider more general rules about how receivers share signals. In this subsection, I let receivers pass on information according to some arbitrary rule, and I study a class of these rules satisfying certain conditions as $n$ gets large. This class of arbitrary sharing rules is more general than the sharing behaviour studied in the main text. 
	
	Given degree sequences, $D$, I append it with a \textit{sharing rule} $\Theta(s) = \{\theta_{i}(s) , \mathbf{d}_{i}(s)\}_{i \in \mathbb{Z} } $ for each signal $s$. The sharing rule captures whether each receiver $i$ shares $s$ and whom she shares $s$ with or hears $s$ from. For each $i$, $\theta_{i}(s)$ is either 0 of 1. If $\theta_{i}(s)=1$, then $i$ shares $s$ and otherwise doesn't. 
	I will refer to $\theta_{i}(s)$ as the \textit{sharing type} and $t_{i}$ as \textit{prior type} of receiver $i$. The degree tuple $\mathbf{d}_{i}$ is a vector $(d_{i}^{t,\theta})_{t \in \{h,l\}, \theta \in \{0,1\} }$ and $d_{i}^{t,\theta}$ is the number of neighbours with type $(t,\theta)$ of receiver $i$. For each $i$ and $t \in \{h,l\}$, $\sum_{\theta} d_{i}^{t,\theta} = d_{i}^{t}$. Therefore, I'll use $d_{i}^{t}$ to refer to both the number of type $t$ neighbours of $i$ as described by degree sequences $D$, and also that implied by sharing rule $\Theta$. Similarly, I use $d_{i}$ to denote the degree of node $i$. 
	
	For a given $D$, I require the sharing rule $\Theta(s)$ for signal $s$ to satisfy some convergence properties. In words, I require that conditional on prior types of a node and its neighbours, the probability that the node shares $s$ converges as $n$ grows. Also, if we in addition condition on sharing type of the node, then as $n$ grows large, the number of its neighbours who have prior type $t$ and share $s$ follows some multinomial distribution. These are stated more formally below:
	\begin{assumption} [\textbf{Convergence of sharing bahaviour} ].
		\begin{enumerate}
			\item There exists a set of real numbers $\{ \hat{\theta}_{t,d}(s) \}_{t \in \{h,l\}, d \in \mathbb{N} }$ all between 0 and 1 such that for all $t \in \{h,l\}$ and $d^{h},d^{l} \in \mathbb{N}$, the ratio
			\[
			\frac{ \sum_{i=1}^{n} \mathbbm{1}(t_{i}=t ,   \theta_{i}(s)=1    ,d_{i}^{h}=d^{h}, d_{i}^{l}=d^{l} )  }{\sum_{i=1}^{n} \mathbbm{1}(t_{i}=t  ,   d_{i}^{h}=d^{h}, d_{i}^{l}=d^{l}       )   }   
			\] 
			converges to $\hat{\theta}_{t,d_{h}+d_{l}}(s)$,	where $\mathbbm{1}(.)$ is the indicator function.
			\item For $t\in \{h,l\}$, define $q_{t}(s) = \sum_{d} \tilde{p}_{d}^{t}\hat{\theta}_{t,d+1}(s)$. For all $t \in \{h,l\}$, $\theta \in \{0,1\}$ and $\mathbf{d} =(d^{t',\theta'})_{t' \in \{h,l \}, \theta' \in \{0,1\} }$, the ratio
			\[
			\frac{ \sum_{i=1}^{n} \mathbbm{1}(t_{i}=t  ,  \theta_{i}(s)=\theta,  \mathbf{d}_{i}=\mathbf{d})  }{\sum_{i=1}^{n} \mathbbm{1}(t_{i}=t  ,  \theta_{i}(s)=\theta , d_{i}^{h}=\sum_{\theta'}d^{h,\theta'} , d_{i}^{l}=\sum_{\theta'}d^{l,\theta'}  )   }  
			\] 
			converges to 
			\[
			Binom(d^{h,1} ;\sum_{\theta'}d^{h,\theta'},q_{h}(s) )
			Binom(d^{l,1} ;\sum_{\theta'}d^{l,\theta'},q_{l}(s) )
			\]
			
			where $Binom(d^{t,\theta'} ;\sum_{\theta'}d^{t,\theta'},q_{t}(s) ) $ is probability that binomial distribution with \\$\sum_{\theta'}d^{t,\theta'}$ trials and success probability $q_{t}(s)$ produces $d^{t,\theta'}$ successes.
		\end{enumerate}
	\end{assumption}
	The assumption is mainly made for analytical tractability. I need some degree of convergence to apply results from random networks. It's nonetheless a reasonable assumption. We are using behaviour when $n$ gets large to capture patterns of behaviour in real world. Since networks and behaviour in real world is obviously not a sequence, it's unclear what a non-convergent sequence in the model means. I also impose the following assumption. 
	\begin{assumption} [\textbf{Believers share more}]
		For all $s \in S$, $ t\in \{h,l\}$ and $d \in \mathbb{N}$, we have $\hat{\theta}_{h,d}(s) \ge \hat{\theta}_{l,d}(s)$
	\end{assumption}
	
	Intuitively, this assumption says that believers would share advertisements or propaganda more than skeptics. This assumption is only required to prove results for networks that exhibit homophily. 
	
	Given degree sequences $D$ and sharing rule $\Theta(s)$, we can append $D$ with the sharing rule $\Theta(s)$ in the following way. For all $D^{(n)}$ and receiver $i$ in $D^{(n)}$, replace $(t_{i}, d_{i}^{l} ,d_{i}^{h})$ with $(t_{i},\theta_{i}(s),\mathbf{d}_{i})$ Note that by our restrictions on $\Theta(s)$, the prior type of $i$ and number of $i$'s neighbours who have prior type $t$ is unchanged by this replacement. We are only adding information about whether $i$ shares signal $s$ and how many of her neighbours would also share signal $s$. This implies that if we ignore the sharing types of nodes, distribution over networks is unchanged by adding these information. Let's denote the appended degree sequences by $D_{\Theta(s)}$. 
	
	The game with $n$ receivers proceeds essentially in the same way as in main text, except that now sender can choose a sharing rule at the beginning and receivers sharing information according to the chosen sharing rule.
	The sender moves first and chooses signal structure, visibility of signals and possibly state dependent seeding strategy. The sender now in addition chooses a sharing rule $\Theta(s)$ for each $s$, from a finite set of sharing rules $\Lambda(s)$ that all satisfy assumptions 2 and 3 above. Receivers observe sender's strategy and chooses their action for all possible observation. Then a signal $s$ and visibility are realised, network is formed according to $D_{\Theta(s)}$ and seeds are selected according to sender's strategy. If $s$ is realised and visible, a receiver observes it iff she's the seed or is connected to a seed by a path of receivers who all share $s$. Payoffs are then realised according to receiver's strategies. Network formation process is still common knowledge, and receivers in addition observe their own degree and prior type. 
	
	I now argue setup in this subsection is indeed more general than setup in the main text. 
	From lemma \ref{lemmanonemptysignalposterior}, we know given any sender's strategy, $s$ must be shared by everyone, by only the believers or by no one. We can imitate these by setting $\theta_{i}(s)=1 $ for all $i$, for all i with $t_{i}=h$ and for no one respectively. It's trivial to check these sharing rules satisfy assumptions 2 and 3. Let $\Lambda(s)$ contain these three rules for all $s$. For any sender's strategy in the main text setup, sender can get exactly the same payoff in the current setup by choosing the same signal structure, visibility and seeding, and choosing sharing rule for each signal $s$ to be what receivers would do in the main text setup. 
	
	Let's now denote sender's payoff by $V^{*}_{net}(D^{(n)},\Lambda )$, since the set of available sharing rules also influence payoffs. 
	We can show that results in the main text extends to this more general setting
	\begin{proposition} \label{proposition4prime}
		If $p_{d}^{h}=p_{d}^{l}$ for all $d$, $q_{h} \ge q_{l}$, and $v$ is convex or linear,\\ $limsup_{n \rightarrow \infty} V^{*}_{net}(D^{(n)},\Lambda ) \le V_{pub}^{*}$.
	\end{proposition}
	\begin{proposition} \label{proposition5prime}
		If $q_{h}=q_{l}$, $\{p_{d}^{h}\}_{d}$ FOSD $\{p_{d}^{l}\}_{d}$, and $v$ is convex or linear,\\ $limsup_{n \rightarrow \infty} V^{*}_{net}(D^{(n)},\Lambda ) \le V_{pub}^{*}$
	\end{proposition}
	
	Since $\Lambda(s)$ is finite, there are finitely many ways to assign a sharing rule for each signal, which is given by the set $\Pi_{s \in S} \Lambda(s)$. I will fix a profile of sharing rule and restrict sender to choose this for all $n$. With this restriction, I can show that limsup of sender's payoff is lower than using public signals. Since there are finitely many possible profiles of sharing rules $\Pi_{s \in S} \Lambda(s)$, this implies that limsup of sender's payoff is lower than using public signals without fixing a profile of sharing rule. 
	
	I first present a few lemmas that are analogous to those used in the main text setup, in order to characterise probabilities that receivers observe each signal. The proofs for these lemmas are essentially the same as those used in the main setup, so some of the details will be omitted. 
	Let $N_{t,\theta, \mathbf{d}}(D_{\Theta(s) } )$ (again, I omit $D_{\Theta(s) }$ unless it may cause confusion) denote the number of receivers with prior type $t$, sharing type $\theta$ for signal $s$, and degree tuple $\mathbf{d} = (d^{t,\theta})_{t \in \{h,l\}, \theta(0,1)}$. Under assumptions 1, 2 and 3, we know that 
	\[
	\frac{N_{t,\theta =1, \mathbf{d}}}{n}
	\]
	converges to 
	\[
	\gamma_{t} \theta_{t,d}(s) p_{d}^{t} Binom(d^{h};d,q_{t}  )Binom(d^{h,1} ; d^{h},q_{h}(s) )Binom(d^{l,1} ; d^{l},q_{l}(s) )
	\]
	Let $\mathbf{q}_{t}$ be the vector $(q_{t}q_{h}(s),q_{t}(1-q_{h}(s)) , (1-q_{t})q_{l}(s), (1-q_{t})(1-q_{l}(s)) )$. Let $MN(d,\mathbf{q} )$ denote the multinomial random variable with $d$ trials, and each type in $\{(h,1),(h,0),(l,1),(l,0) \}$ realises with probability given by respective element in $\mathbf{q}_{t}$. One can show that 
	\[
	Binom(d^{h};d,q_{t}  )Binom(d^{h,1} ; d^{h},q_{h}(s) )Binom(d^{l,1} ; d^{l},q_{l}(s) ) = Pr(MN(d,\mathbf{q}_{t} ) = \mathbf{d} )
	\]
	Also, we can rearrange $\gamma_{t} \theta_{t,d}(s) p_{d}^{t}$ to be $ \gamma_{t} \sum_{d'} \theta_{t,d'}(s) p_{d'}^{t} \frac{\theta_{t,d}(s) p_{d}^{t} }{ \sum_{d'} \theta_{t,d'}(s) p_{d'}^{t} }$. In words, the proportion of receivers who have type $(t,1)$ converges to $ \gamma_{t} \sum_{d'} \theta_{t,d'}(s) p_{d'}^{t}$. Conditional on having type $(t,1)$, the degree distribution is given by $\frac{\theta_{t,d}(s) p_{d}^{t} }{ \sum_{d'} \theta_{t,d'}(s) p_{d'}^{t} }$. Conditional on having type $(t,1)$ and degree $d$, the distribution over types of these $d$ neighbours is given by the multinomial random variable $ MN( d,\mathbf{q}_{t}) $. Therefore, the appended degree sequences $D_{\Theta(s)}$ satisfy conditions imposed on degree sequences in \citet{sadler2020}, (which is a generalised version of assumption 1 allowing for more than 2 types). We can apply results on random networks in it. 
	
	To state and use these results, we need to define some branching processes again. For the sake of space, I'll omit a formal description, since it's very similar to the ones stated in subsection 6.2 in appendix. Let $p_{d}^{t,\theta}$ denote the degree distribution of receivers with type $(t,\theta)$. Let $\tilde{p}_{d}^{t,\theta}$ denote the forward distribution for $p_{d}^{t,\theta}$. Let $\tilde{\mathcal{B}}(D_{\Theta(s)} | t,\theta ) $ denote the branching process that have an initial node of type $(t,\theta)$ in generation 1. Each node in generation $\tau$ produces generation $\tau+1$ offsprings according to degree distribution $p_{d}^{t,\theta}$. Conditional on having $d$ offsprings, the types of them is determined by $MN(d,\mathbf{q}_{t})$. All nodes produce offsprings mutually independently of each other. 
	
	Another branching process $\mathcal{B}(D_{\Theta(s)})$ is defined as the branching process with one node in generation 1. That node has each type $(t,\theta=1)$ with probability $\gamma_{t} \sum_{d'} \theta_{t,d'}(s) p_{d'}^{t}$ and each $(t,\theta=0)$ with probability $\gamma_{t} (1-\sum_{d'} \theta_{t,d'}(s) p_{d'}^{t})$. Given its type $(t,\theta)$, it produces offsprings according to $p_{d}^{t,\theta}$. From next generation onwards, the branching process behaves in the same way as any $\tilde{\mathcal{B}}(D_{\Theta(s)} | t,\theta ) $. 
	
	I use $\rho^{1}_{D_{\Theta(s)}} (m)$ and $\tilde{\rho}^{1}_{D_{\Theta(s)}}(m | t, \theta)$ to denote the probability that branching processes $\mathcal{B}(D_{\Theta(s)}) $ and $\tilde{\mathcal{B}} (D_{\Theta(s)}|t,\theta)$ contains less than $m$ nodes after deleting nodes with ancestors who doesn't share $s$ except the root node. Similarly, let $\rho^{1}_{D_{\Theta(s)}} (\infty)$ and $\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, \theta)$ denote the probability that the respective branching processes never die out, after deleting nodes with ancestors who doesn't share $s$ except the root node. Proof for remark 2 still goes through, and we have $\rho^{1}_{D_{\Theta(s)}} (\infty)= 1- \lim_{m \rightarrow \infty} \rho^{1}_{D_{\Theta(s)}} (m)$ and $\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, \theta) =1- \lim_{m \rightarrow \infty} \tilde{\rho}^{1}_{D_{\Theta(s)}} (m|t, \theta)$. 
	
	We also know that, for all these branching processes, conditional having $d^{h,1}$ offsprings with type $(h,1)$ and $d^{l,1}$ offsprings with type $(l,1)$ in generation 2, the probability that the process never dies out after deleting nodes with ancestors who doesn't share $s$ except the root node is 
	\[
	1-    (1- \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1))^{d^{h,1}}   (1-  \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1))^{d^{l,1}}
	\]
	The proof is essentially the same as that for remark 3. In short, the whole process never dies out if and only if the process that branches from at least one of the generation 1 nodes never dies out. 
	By construction, the process that branches from a node of type $(t, \theta)$ in generation 1 is identical to the branching process $\tilde{\mathcal{B}} (D_{\Theta(s)}|t,\theta)$. Also, all the nodes produce offsprings mutually independently from each other, so processes branching from the generation 1 nodes are all mutually independent of each other. The equality above follows. 
	
	Let $N^{1}_{t,d,m}(g^{n})$ denote the number of nodes that have prior type $t$, degree $d$ and is connected to less than $m$ nodes after deleting all nodes with sharing type 0. Let $N_{t,d}$ denote the number of nodes that have prior type $t$, degree $d$ as before. Let $\hat{L}_{i}^{s}$ denote $i$-th largest component after deleting nodes with sharing type 0. Applying proposition 10 from \citet{sadler2020} gives the following result
	\begin{lemma} \label{lemmaextensionbranchmatch}
		For any $t \in \{h,l\}$, $d,m \in \mathbb{N}$, we have that $\frac{N^{1}_{t,d,m}(g^{n})}{N_{t,d}}$ converges in probability to $\rho^{1}_{D_{\Theta(s)}} (m | t,d)$, where $\rho^{1}_{D_{\Theta(s)}} (m | t,d)$ is the probability that branching processes $\mathcal{B}(D_{\Theta(s)}) $ contains less than $m$ nodes after deleting nodes with ancestors (except root node) who doesn't share $s$ conditional on root node having prior type $t$ and $d$ offsprings. 
	\end{lemma}
	
	Using this lemma, we can obtain the following lemma on the probability that a node is on giant component. Let $N^{1}_{t,d,\hat{L}_{i}^{s} }(g^{n})$ denote the number of nodes that have prior type $t$, degree $d$ and has a neighbour on $\hat{L}_{i}^{s}$.
	\begin{lemma} \label{lemmaextensionongiant}
		For any $t \in \{h,l\}$, $d \in \mathbb{N}$, $\frac{N^{1}_{t,d,\hat{L}_{i}^{s} } (g^{n})}{N_{t,d}}$ converges in probability to $\rho^{1}_{D_{\Theta(s)}} (\infty | t,d)$, where $\rho^{1}_{D_{\Theta(s)}} (\infty | t,d)$ is the probability that branching processes $\mathcal{B}(D_{\Theta(s)}) $ never dies out after deleting nodes with ancestors (except root node) who doesn't share $s$, conditional on root node having prior type $t$ and $d$ offsprings. 
	\end{lemma}
	
	Let $\hat{\zeta}^{s}(t,d)$ denote $\rho_{D_{\Theta(s)}}^{1}(\infty| t,d)  $.
	Define $\hat{C}^{s}_{1}(.)$ to be a function
	\[
	\hat{C}^{s}_{1}(z,g^{n}) =  \begin{cases}
		1 & \text{ if at least one of $z$ is on $\hat{L}^{s}_{1}$ of $g^{n}$} \\
		0 & \text{otherwise}
	\end{cases}
	\]
	Define $\mathcal{A}^{s}_{n}(\alpha, \overline{d})$ to be the set of networks with $n$ receivers that satisfy the following property: Given any sender's strategy $\Pi^{n}$ in the network signal game with $n$ receivers, for each $s \in S$, given that network $g^{n} \in \mathcal{A}^{s}_{n}(\alpha,\overline{d})$, signal $s$ and seeds $z$ are realised and $s$ is visible, the proportion of receivers with prior type $t$ and degree $d \le \overline{d}$ who observe $s$ is in the range
	\[ [\hat{C}^{s}_{1}(z,g^{n})\hat{\zeta}^{s}(t,d) + \alpha, \hat{C}^{s}_{1}(z,g^{n})\hat{\zeta}^{s}(t,d) - \alpha]  \]
	
	
	\begin{lemma} \label{lemmaextensionobservesignal}
		Given any $D_{\Theta(s)}$, $\overline{d} \in \mathbb{N}$ and $\alpha,\epsilon > 0$, there exists an $n_{1}$ large enough such that for any $n \ge n_{1}$, $Pr(g^{n} \in \mathcal{A}^{s}_{n}(\alpha,\overline{d} )   ) > 1-\epsilon$
	\end{lemma}
	
	Proof of the previous two lemmas are essentially the same as proofs for \ref{lemmaprobongiant} and \ref{lemmaobservesignal} and thus are omitted. Detailed roofs are available from the author. 
	
	\begin{lemma} \label{lemmaextensionbelieversobservemore}
		If $p_{d}^{h}=p_{d}^{l}$, then for any $d$, $\rho_{D_{\Theta(s)}}^{1} (\infty| h,d) \ge \rho_{D_{\Theta(s)}}^{1}(\infty|l,d)$. Therefore, using notations above, we have $\hat{\zeta}^{s}(h,d) \ge \hat{\zeta}^{s}(l,d)  $
	\end{lemma}
	\begin{proof}
		I use $p_{d}$ to denote both $p_{d}^{h}$ and $p_{d}^{l}$ since they are equal. 
		
		For branching process $ \mathcal{B}(D_{\Theta(s)})$, conditional on the root node having prior type $t$, the probability that it produces $d$ offsprings is given by 
		\[
		{ \sum_{d'} \theta_{t,d'}(s) p_{d'} } \frac{ \theta_{t,d}(s) p_{d} }{ \sum_{d'} \theta_{t,d'}(s) p_{d'} } + (1-{ \sum_{d'} \theta_{t,d'}(s) p_{d'} }) \frac{  (1-\theta_{t,d}(s)) p_{d} } {1- { \sum_{d'} \theta_{t,d'}(s) p_{d'} }} = p_{d}
		\]
		Also, we know that conditional on the root node having type $(t,\theta)$ and $d$ offsprings, the types of its offsprings are determined by the multinomial distribution $MN(d,\mathbf{q}_{t})$. Since $\mathbf{q}_{t}$ doesn't depend on sharing type $\theta$, conditional on the root node having prior type $t$ and $d$ offsprings, the types are still determined by $MN(d,\mathbf{q}_{t})$. Therefore, the probability that condtiional on root node having prior type $t$, the probability that it never dies out is
		\[
		\sum_{d} p_{d} \sum_{\mathbf{d}} Pr(MN(d,\mathbf{q}_{t}) = \mathbf{d})  (1-    (1- \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1))^{d^{h,1}}   (1-  \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1))^{d^{l,1}})
		\]
		After some rearrangement, one can show that this is equal to
		\[
		1- \sum_{d} p_{d}  (1-    q_{t}q_{h}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1)   -    (1-q_{t})q_{l}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1) )^{d}
		\]
		Similarly, for the branching process $\tilde{\mathcal{B}}(D_{\Theta}(s)| t,\theta=1)$, the probability that the process never dies out is
		\[
		\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, 1) = \sum_{d} \frac{\theta_{t,d+1}p_{d+1}(d+1)}{ \sum_{d'} \theta_{t,d'}p_{d'}d' } \sum_{\mathbf{d}} Pr(MN(d,\mathbf{q}_{t}) = \mathbf{d})  (1-    (1- \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1))^{d^{h,1}}   (1-  \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1))^{d^{l,1}})
		\]
		and can be rearranged to get
		\[
		\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, 1) = 1- \sum_{d} \frac{\theta_{t,d+1}p_{d+1}(d+1)} { \sum_{d'} \theta_{t,d'}p_{d'}d' }  (1-    q_{t}q_{h}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1)   -    (1-q_{t})q_{l}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1) )^{d}
		\]
		Note that $q_{t}(s)$ is equal to 
		\[
		\sum_{d} \frac{(d+1)p_{d+1} \theta_{t,d+1}(s)}{\sum_{d'} d'p_{d'}}
		\]
		by construction. If we multiply both sides by $q_{t}(s)$, we get
		\[
		q_{t}(s)\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, 1) = q_{t(s)}  -  \sum_{d} \tilde{p}_{d}\theta_{t,d+1}(s)  (1-    q_{t}q_{h}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1)   -    (1-q_{t})q_{l}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1) )^{d}
		\]
		After some rearranging, we get
		\[
		q_{t}(s)( 1- \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | t, 1)) = \sum_{d} \tilde{p}_{d}\theta_{t,d+1}(s)  (q_{t} (1-  q_{h}(s) \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1))   +    (1-q_{t}) (1- q_{l}(s)\tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1) )^{d})
		\]
		
		Therefore, we know that $x =  \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | h, 1)$ and $ y =  \tilde{\rho}^{1}_{D_{\Theta(s)}}(\infty | l, 1)$ must be a solution to the following system of equations
		\[
		q_{h}(s)(1-x) = \sum_{d} \tilde{p}_{d}\theta_{h,d+1}(s)  (q_{h} (1- q_{h}(s)x)   +    (1-q_{h})(1-q_{l}(s)y) )^{d}
		\]
		\[
		q_{l}(s)(1-y) = \sum_{d} \tilde{p}_{d}\theta_{l,d+1}(s)  ( q_{l} (1 - q_{h}(s)x)   +    (1-q_{l}) (1-q_{l}(s)y))^{d}
		\]
		I now argue that there can exist no solution to this system of equations such that $x < y$. Suppose there exists such a solution $(x_{1},y_{1})$. From our condition that $\theta_{h,d}(s) \ge \theta_{l,d}(s)$, one can verify that $q_{h}(s) \ge q_{l}(s)$ and the degree distribution $\{\tilde{p}_{d}\theta_{h,d+1} \}_{d}$ FOSD $\{\tilde{p}_{d}\theta_{l,d+1} \}_{d}$. Since we know that 
		\[
		q_{l}(s)(1-y_{1}) = \sum_{d} \tilde{p}_{d}\theta_{l,d+1}(s)  ( q_{l} (1 - q_{h}(s)x_{1})   +    (1-q_{l}) (1-q_{l}(s)y_{1}))^{d}
		\]
		we have that 
		\[
		q_{h}(s)(1-y_{1}) > \sum_{d} \tilde{p}_{d}\theta_{h,d+1}(s)  ( q_{h} (1 - q_{h}(s)y_{1})   +    (1-q_{h}) (1-q_{l}(s)y_{1}))^{d}
		\]
		Let's define $f_{lhs} (x) = q_{h}(s)(1-x)$ and $f_{rhs}(x) = \sum_{d} \tilde{p}_{d}\theta_{h,d+1}(s)  (q_{h} (1- q_{h}(s)x)   +    (1-q_{h})(1-q_{l}(s)y_{1}) )^{d}$. We know that $f_{lhs}(y_{1}) > f_{rhs}(y_{1})$. We also know that $f_{lhs} (0) = q_{h}(s)$ and 
		\[
		f_{rhs}(0) = \sum_{d} \tilde{p}_{d}\theta_{h,d+1}(s)  (q_{h}   +    (1-q_{h})(1-q_{l}(s)y_{1}) )^{d} < \sum_{d} \tilde{p}_{d}\theta_{h,d+1}(s) = q_{h}(s) = f_{lhs}(1)
		\]
		Since $f_{lhs} (x)$ is linear and $f_{rhs} (x)$ is convex, $f_{lhs} (y_{1}) >f_{rhs} (y_{1})$ and $f_{lhs} (0) >f_{rhs} (0)$, there can't exist some $x \in [y_{1} , 1]$ that solves $f_{lhs} (x) =f_{rhs} (x)$. This is a contradiction that $x_{1}<y_{1}$ solves this equation. This concludes the proof. 
	\end{proof}
	Let $\Pi^{n}$ be some sender's strategy in the game with $n$ receivers. Define $\hat{V}^{ext}(d,\Pi^{n})$ as follows
	\begin{multline} \label{vhatextension}
		\hat{V}^{ext}(d,\Pi^{n}  ) \equiv 	
		\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi(s|\omega)\bigg[  (1-b(\omega))  v\big(\sum_{t}\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n})\big) +\\
		b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}) \\
		\bigg(
		v\big(\sum_{t} \frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\gamma_{t}\alpha(s,t,d;\Pi^{n})+ (1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n})\big)  \bigg) 
		\bigg]  
	\end{multline}
I show the following lemma.
\begin{lemma} \label{lemmavhatexten}
	Suppose that $\hat{ \zeta }^{s}(h,d) \ge \hat{\zeta}^{s}(l,d)$ for all $s$ and $d$. 
	If $v$ is linear or convex, for any $\beta>0$ and $d$, there exists $n_{1}$ such that for all $n \ge n_{1}$, then $\hat{V}^{ext}(d,\Pi^{n}  ) \le V_{pub}^{*}+ \beta$ for all possible sender's strategy. 
\end{lemma}
\begin{proof}
	For any $\beta'>0$, we can find a $\beta>0$ such that $\sup_{x \in [0,1]}( v(x+4\beta)-v(x)) < \beta'$.  We can find some $n_{1}$ such that for all $n>n_{1}$, we have $Pr(g^{n} \in \mathcal{A}^{s}_{n}(\beta,\overline{d} )  ) > \beta$ for all $s \in S$. 

Denote the set of signals $s$ with $\alpha(s,l,d;\Pi^{n}) =1$ by $S_{good}$, and the set of signals with $\alpha(s,l,d;\Pi^{n}) =0$ and $\alpha(s,h,d;\Pi^{n}) =1$ by $S_{int}$, and the rest of the signals by $S_{bad}$. 
	We consider two cases. First, suppose that $\alpha(\emptyset,l,d;\Pi^{n}) = 0$. By property of $Pr(g^{n} \in \mathcal{A}^{s}_{n}(\beta,\overline{d} )  )$, We can get an upper bound of $\hat{V}^{n}(d,\Pi^{n}  )$ as
\begin{multline} \label{expropeq37}	
	\beta v(1) + \sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi(s|\omega)\bigg[  (1-b(\omega))  v\big(\sum_{t}\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n})\big) +\\
	b(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}) \\
	\bigg(
	v\big(2\beta + \sum_{t} \frac{N_{h,d,s}(g^{n},z)}{N_{h,d}}\gamma_{t}\alpha(s,t,d;\Pi^{n})+ (1-\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}})\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n})\big)  \bigg) 
	\bigg]  
\end{multline}
This by convexity of $v$ and definition of $\beta$ is smaller than
\begin{multline} \label{expropeq8}	
	  \sum_{\omega} \mu_{s}(\omega)\bigg[
	\bigg( 1-b(\omega)  + b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})                          \bigg)v\big(\gamma_{h}\alpha(\emptyset,t,d;\Pi^{n})\big) \\
	+b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}}v(1)      \\
	+b(\omega) \sum_{s \in S_{int}}                 \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}}v(\gamma_{h})            
	\bigg] + \beta v(1) + \beta'
\end{multline}
Consider sender's public signal strategy $(\pi_{2},b_{2})$ described as follows: For $\omega \in \{0,1\}$, 
\[
b_{2}(\omega) = b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}
\]
For $j \in \{good,int,bad\}$ and $\omega=1$
\[
\pi_{2}(s_{j}|\omega=1) = \frac{b(\omega=1)\sum_{s \in S_{j}} \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}}{b_{2}(\omega=1)}
\]
For $s_{good}$, set 
\begin{multline}
	\pi_{2}(s_{good}|\omega=0 ) =min\{ \frac{b_{2}(\omega=1)\pi_{2}(s_{good}|\omega=1) \mu_{l}(\omega=1) }{ b_{2}(\omega=0) \mu_{l}(\omega=0)  } ,  \\ \frac{b(\omega=0)\sum_{s \in S_{good}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	}}{b_{2}(\omega=0)}    \} 
\end{multline}
For $s_{int}$, set 
\[
\pi_{2}(s_{int}|\omega=0 ) = \frac{b(\omega=0)\sum_{s \in S_{int}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}}{b_{2}(\omega=0)} \]
One can verify that $\pi_{2}(s_{int}|\omega=0 ) + \pi_{2}(s_{good}|\omega=0 ) \le 1$. For $s_{bad}$, set 
\[
\pi_{2}(s_{bad}|\omega=0) = 1- \pi_{2}(s_{int}|\omega=0 ) - \pi_{2}(s_{good}|\omega=0 )
\]

By construction, we know that all receivers must choose action 1 upon observing $s_{good}$. Also, similar to the proof in proposition \ref{baselineprop}, one can verify that type $h$ receivers will choose action 1 upon observing $s_{int}$. We know that for all $s \in S_{good}$,

\begin{multline}
	\mu_{l}(\omega=1) b(\omega=1) \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}   \\ \ge \mu_{l}(\omega=0) b(\omega=0) \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}
\end{multline}

Therefore

\begin{multline}
	2\beta+\mu_{l}(\omega=1) b(\omega=1) \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\hat{C}^{s}_{1}(z,g^{n})\hat{\zeta}^{s}(l,d)
 \\
 \ge -2\beta + \mu_{l}(\omega=0) b(\omega=0)\pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\hat{C}^{s}_{1}(z,g^{n})\hat{\zeta}^{s}(l,d)
\end{multline}
If $\hat{\zeta}^{s}(l,d) \ne 0$, this in turn implies that  
\begin{multline}
	2(\frac{\hat{\zeta}^{s}(h,d)}{\hat{\zeta}^{s}(l,d)}+1)\beta+\mu_{l}(\omega=1) b(\omega=1)\pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	}   \\
 \ge -2(\frac{\hat{\zeta}^{s}(h,d)}{\hat{\zeta}^{s}(l,d)}+1)\beta + \mu_{l}(\omega=0) b(\omega=0) \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}
\end{multline}
Let $K_{3}$ denote the largest $\frac{\hat{\zeta}^{s}(h,d)}{\hat{\zeta}^{s}(l,d)}$ for all $s \in S_{good}$ and $\hat{\zeta}^{s}(l,d) \ne 0$. Summing the inequality above over all $s \in S_{good}$, we get
\begin{multline}
	\mu_{l}(\omega=1) b(\omega=1)\sum_{s \in S_{good}}\pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	}   \\
	\ge -4|S|(K_{3}+2)\beta + \mu_{l}(\omega=0) b(\omega=0) \sum_{s \in S_{good}}\pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	}
\end{multline}
By definition, this implies
\begin{multline}
	\pi_{2}(s_{good}|\omega =0)b_{2}(\omega=0) \ge  b(\omega=0)\sum_{s \in S_{good}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	} \\ -4|S|(K_{3}+2)\beta/\mu_{l}(\omega=0)
\end{multline}
Also, receivers observe $\emptyset$ with the same probability as receivers with prior type $t$ and degree $d$ under network signal strategy $\Pi_{1}^{n}$. Therefore, type $h$ receivers must choose action 1 upon observing $\emptyset$ under public signal strategy $(\pi_{2},b_{2})$ defined above. 

Combining these facts, sender's payoff using $(\pi_{2},b_{2})$ is at least
\begin{multline} \label{expropeq9}	
	\sum_{\omega} \mu_{s}(\omega)\bigg[
	\bigg( 1-b(\omega)  + b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})                          \bigg)v\big(\gamma_{h}\alpha(\emptyset,t,d;\Pi^{n})\big) \\
	+b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}}v(1)      \\
	+b(\omega) \sum_{s \in S_{int}}                 \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}}v(\gamma_{h})            
	\bigg] -4v(1)|S|(K_{3}+2)\beta/\mu_{l}(\omega=0)
\end{multline}
Proof for the first case follows since $\beta$ can be arbitrarily small.

Now we consider the second case. Suppose that $\alpha(\emptyset,l,d;\Pi^{n}) = 1$. We can bound $\hat{V}^{n}(d,\Pi^{n}  )$ above by
\begin{multline}
\beta v(1) +	\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi(s|\omega)\bigg[  (1-b(\omega))  v\big(1\big) +\\
	b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}) 
	\bigg(
	v\big(2\beta + \sum_{t} \frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}\gamma_{t}\alpha(s,t,d;\Pi^{n})+ (1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})\gamma_{t}\big)  \bigg) 
	\bigg]
\end{multline}
By convexity, this is smaller than
\begin{multline} \label{expropeq10}	
	\sum_{\omega} \mu_{s}(\omega)\bigg[
	\bigg( 1-b(\omega)  + b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})(1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})                          \bigg)v\big(1\big) \\
	+b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}v(1)      \\
	+b(\omega) \sum_{s \in S_{int}}                 \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}v(\gamma_{h})            
	\bigg] +\beta' + \beta v(1)
\end{multline}

Consider sender's public signal strategy $(\pi_{3},b_{3})$ described as follows:
\[
b_{3}(\omega) = b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}
\]
For $j \in \{good,int,bad\}$ and $\omega=1$
\[
\pi_{3}(s_{j}|\omega=1) = \frac{b(\omega=1)\sum_{s \in S_{j}} \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}}{b_{3}(\omega=1)}
\]
For $s_{int}$, set 
\begin{multline}
	\pi_{3}(s_{int}|\omega=0 ) =min\{ \frac{b_{3}(\omega=1)\pi_{3}(s_{int}|\omega=1) \mu_{l}(\omega=1) }{ b_{3}(\omega=0) \mu_{l}(\omega=0)  } ,  \\ \frac{b(\omega=0)\sum_{s \in S_{int}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
	}}{b_{3}(\omega=0)}    \} 
\end{multline}
For $s_{good}$, set 
\[
\pi_{3}(s_{good}|\omega=0 ) = \frac{b(\omega=0)\sum_{s \in S_{good}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}}{b_{3}(\omega=0)} \]
One can verify that $\pi_{3}(s_{int}|\omega=0 ) + \pi_{3}(s_{good}|\omega=0 ) \le 1$. For $s_{bad}$, set 
\[
\pi_{3}(s_{bad}|\omega=0) = 1- \pi_{3}(s_{int}|\omega=0 ) - \pi_{3}(s_{good}|\omega=0 )
\]
By essentially the same argument as in the previous case, all receivers choose action 1 upon observing signal $s_{good}$ with the public signal structure $(\pi_{3},b_{3})$. Similarly, type $h$ receivers choose action 1 upon observing $s_{int}$.

Also, receivers observe $\emptyset$ in each state with the same probability as that of a receiver with type $l$ and degree $d$ under network signal structure $\Pi^{n}$. Therefore, all receivers must choose action 1 upon observing $\emptyset$. We know that for all $s \in S_{int}$
\begin{multline}
	\mu_{h}(\omega=1) b(\omega=1) \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}\ge \\
 \mu_{h}(\omega=0) b(\omega=0) \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
}
\end{multline}

Using similar arguments as above, if $\hat{\zeta}^{s}(h,d) \ne 0$ ,this inequality implies that
\begin{multline}
2(1 + \frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)})\beta+ \mu_{h}(\omega=1) b(\omega=1) \pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
} \ge  \\
 - 2(1 + \frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)})\beta + \mu_{h}(\omega=0) b(\omega=0) \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
}
\end{multline}
Let $K_{4}$ denote the largest value of $\frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)}$ among all $s \in S_{int}$.
Summing over all signals $s \in S_{int}$ implies that
\begin{multline}
 \mu_{h}(\omega=1) b(\omega=1) \sum_{s \in S_{int}}\pi(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
	} \ge  \\
	- 4(2 + \frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)})\beta + \mu_{h}(\omega=0) b(\omega=0) \sum_{s \in S_{int}}\pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
	}
\end{multline}
By construction, this implies that
\begin{multline}
	\pi_{3}(s_{int}|\omega=0)b_{3}(\omega=0) \ge   \\ b(\omega=0)\sum_{s \in S_{int}} \pi(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
	} -\frac{4(2 + \frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)})\beta}{\mu_{h}(\omega=0)}
\end{multline}
Using this inequality these, sender's payoff using $(\pi_{3},b_{3})$ is at least
\begin{multline} \label{expropeq11}	
	\sum_{\omega} \mu_{s}(\omega)\bigg[
	\bigg( 1-b(\omega)  + b(\omega)\sum_{s \in S} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})(1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})                          \bigg)v\big(1\big) \\
	+b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}v(1)      \\
	+b(\omega) \sum_{s \in S_{int}}                 \pi(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}v(\gamma_{h})            
	\bigg]  -\frac{4(2 + \frac{\hat{\zeta}^{s}(l,d)}{\hat{\zeta}^{s}(h,d)})\beta}{\mu_{h}(\omega=0)}v(1)
\end{multline}

The result follows since $\beta$ and $\beta'$ can be arbitrarily small and $v(.)$ is bounded.
\end{proof}
	
	We are now ready to prove propositions \ref{proposition4prime} and \ref{proposition5prime} 
	
		\textit{Proof of proposition \ref{proposition4prime} :}\\
		Since two types have the same degree distribution, I again use $p_{d}$ to denote both of them. 
		
		For any $\beta'>0$, we can find a $\beta>0$ such that $\sup_{x \in [0,1]}( v(x+4\beta)-v(x)) < \beta'$. For this $\beta$, we can find some $\overline{d}$ such that $\sum_{d>\overline{d}} p_{d}	 <\beta $. Fix this $\overline{d}$. By lemmas above and construction, we can find some $n_{1}$ such that for all $n>n_{1}$, the following conditions are satisfied:
		\begin{enumerate}
			\item $\sum_{d > \overline{d}}  \frac{N_{h,d}+N_{l,d}}{n}  < \beta  $
			\item $\frac{N_{t,d}}{n}  \in [\gamma_{t}p_{d}(1-\beta) ,  \gamma_{t}p_{d} (1+ \beta)]  $ for $t\in \{h,l\}$ and all $d \le \overline{d}$. 
			\item  $\hat{V}^{ext}(d,\Pi^{n}  ) \le V_{pub}^{*}+ \beta$ for all possible sender's strategy and $d \le \overline{d}$ if $v$ is convex or linear.
		\end{enumerate}
		
		Let $N_{t,d,s}(g^{n},z)$ denote the number of prior type $t$ degree $d$ receivers that observe signal $s$, given network $g^{n}$, seeds $z$ and signal $s$ being realised and visible. 
		In the game with $n$ receivers, sender's payoff from some network signal strategy $\Pi^{n}_{1}$ is given by
		\begin{multline} \label{expropeq1}
			\sum_{\omega} \mu_{s}(\omega)\sum_{s \in S} \pi_{1}(s|\omega)\bigg[  (1-b_{1}(\omega)) v(\sum_{t,d}\frac{N_{t,d}}{n} \alpha(\emptyset,t,d;\Pi^{n}_{1})) +\\
			b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}_{1}) v(\sum_{t,d}\frac{N_{t,d,s}(g^{n},z)}{n}\alpha(s,t,d;\Pi^{n}_{1}) +  (1-\frac{N_{t,d,s}(g^{n},z)}{n})\alpha(\emptyset,t,d;\Pi^{n}_{1})  )    
			\bigg]
		\end{multline}
		where $b_{1}$ and $\pi_{1}$ are sender's signal structure and visibility in $\Pi^{n}_{1}$. Using steps essentially the same as those used in proof of proposition 1 and 4, \ref{expropeq1} is bounded above by. 
		\begin{multline} \label{expropeq5}
			\sum_{d \le \overline{d}}p_{d}
			\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi_{1}(s|\omega)\bigg[  (1-b_{1}(\omega))  v\big(\sum_{t}\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
			b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}_{1}) \\
			\bigg(
			v\big(\sum_{t} \frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\gamma_{t}\alpha(s,t,d;\Pi^{n}_{1})+ (1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\gamma_{t}\alpha(\emptyset,t,d;\Pi^{n}_{1})\big)  \bigg) 
			\bigg]   + \beta'
		\end{multline}
		which by definition is equal to $\sum_{d \le \overline{d}}p_{d} \hat{V}^{ext}(d,\Pi^{n}_{1}) + \beta'$. By point 3 in conditions at the beginning of the proof, $\sum_{d \le \overline{d}}p_{d} \hat{V}^{ext}(d,\Pi^{n}_{1}) + \beta' \le V_{pub}^{*} + \beta +\beta'$. The proposition follows since $\beta$ and $\beta'$ can be arbitrarily small. 
	\qed
	
	
	\textit{Proof of proposition \ref{proposition5prime} }:\\
		Since $q_{h} = q_{l}$, we know that $\hat{\zeta}^{s}(h,d)=\hat{\zeta}^{s}(l,d)$, for all $s$, so I omit arguments of type in $\hat{\zeta}^{s}$. 
		
		For any $\beta'>0$, we can find a $\beta>0$ such that $sup( v(x+8\beta)-v(x)) < \beta'$. For this $\beta$, we can find some $\overline{d}$ such that $\sum_{d>\overline{d}} (p_{d}^{h}+p_{d}^{l}	) <\beta $. Fix this $\overline{d}$. By lemmas above and construction, we can find some $n_{1}$ such that for all $n>n_{1}$, the following conditions are satisfied:
		\begin{enumerate}
			\item $\sum_{d > \overline{d}}  \frac{N_{h,d}+N_{l,d}}{n}  < \beta  $
			\item $\frac{N_{t,d}}{n}  \in [\gamma_{t}p_{d}(1-\beta) ,  \gamma_{t}p_{d} (1+ \beta)]  $ for $t\in \{h,l\}$ and all $d \le \overline{d}$. 
			\item $Pr(g^{n} \in \mathcal{A}^{s}_{n}(\beta,\overline{d} )  ) > 1-\epsilon$ for all $s$.
			\item  $\hat{V}^{ext}(d,\Pi^{n}  ) \le V_{pub}^{*}+ \beta$ for all possible sender's strategy and $d \le \overline{d}$ if $v$ is convex or linear.
		\end{enumerate}
		For any $n \ge n_{1}$ and sender's strategy $\Pi^{n}_{1}$.
		
		Also, let $N_{t,d,s}(g^{n},z)$ denote the number of type $t$ degree $d$ receivers that observe signal $s$, given network $g^{n}$, seeds $z$ and signal $s$ being realised and visible.
		
		In the game with $n$ receivers, by essentially the same steps as in the proof of proposition 1 and 4, sender's payoff from $\Pi^{n}_{1}$ is bounded above by,
		\begin{multline} \label{exprop3eq1}
		Pr((g^{n} \in \mathcal{A}^{s}_{n}(\beta,\overline{d} ) )	\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi_{1}(s|\omega)\bigg[  (1-b_{1}(\omega)) v\big(2\beta+\sum_{t,d \le \overline{d} }\gamma_{t}p_{d}^{t} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
			b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n}|(g^{n} \in \mathcal{A}^{s}_{n}(\beta,\overline{d} ))Pr(z|s,g^{n},\omega;\Pi^{n}_{1}) \\
			v\big(2\beta + \sum_{t,d \le \overline{d} }p_{d}^{t}\gamma_{t}
			\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\alpha(s,t,d;\Pi^{n}_{1}) +  p_{d}^{t}\gamma_{t}(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\alpha(\emptyset,t,d;\Pi^{n}_{1})   \big) 
			\bigg]  
			+ \beta v(1)
		\end{multline}
		Again, we consider two cases. In the first case, suppose that $\alpha(\emptyset, l, d ;\Pi_{1}^{n}) =0 $ for all $d \le \overline{d}$. In this case, by definition, we know that 
		\[
		\sum_{d \le \overline{d} }\gamma_{t}p_{d}^{l} \alpha(\emptyset,l,d;\Pi^{n}_{1}) = \sum_{d \le \overline{d} }\gamma_{t}p_{d}^{h} \alpha(\emptyset,l,d;\Pi^{n}_{1})
		\]
		From properties of $\mathcal{A}^{s}_{n}(\beta,\overline{d})$, we know that for any $s \in S$, $d_{1},d_{2} \le \overline{d}$ and $d_{1} \le d_{2}$, we have  
		\[
		\frac{N_{l,d_{1},s}(g^{n},z)}{N_{l,d_{1}}} - \frac{N_{l,d_{2},s}(g^{n},z)}{N_{l,d_{2}}} \le 2\beta
		\]
		Therefore, since $p_{d}^{h}$ FOSD $p_{d}^{l}$, for any $s \in S_{good}$, $d_{1},d_{2} \le \overline{d}$ and $d_{1} \le d_{2}$,
		\begin{multline}
			2\beta+	\sum_{d \le \overline{d} }p_{d}^{h}\gamma_{l}
			\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}\alpha(s,l,d;\Pi^{n}_{1}) +  p_{d}^{h}\gamma_{l}(1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})\alpha(\emptyset,l,d;\Pi^{n}_{1}) \ge  \\
			\sum_{d \le \overline{d} }p_{d}^{l}\gamma_{l}
			\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}\alpha(s,l,d;\Pi^{n}_{1}) +  p_{d}^{l}\gamma_{l}(1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})\alpha(\emptyset,l,d;\Pi^{n}_{1})
		\end{multline}
		Therefore, expression \ref{exprop3eq1} is bounded above by
		\begin{multline} \label{exprop3eq2}
			\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi_{1}(s|\omega)\bigg[  (1-b_{1}(\omega)) v\big(2\beta+\sum_{t,d \le \overline{d} }\gamma_{t}p_{d}^{h} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
			b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}_{1}) \\
			v\big(2\beta+2\beta + \sum_{t,d \le \overline{d} }p_{d}^{h}\gamma_{t}
			\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\alpha(s,t,d;\Pi^{n}_{1}) +  p_{d}^{h}\gamma_{t}(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\alpha(\emptyset,t,d;\Pi^{n}_{1})   \big) 
			\bigg]  
			+ \beta v(1)
		\end{multline}
		By convexity and definition of $\beta$, \ref{exprop3eq2} is smaller than (after some rearrangement)
		\[\sum_{d \le \overline{d}}p_{d}^{h} \hat{V}^{ext}(d,\Pi^{n}_{1}) + \beta v(1) + \beta' \le  V_{pub}^{*}+ \beta v(1) + \beta'+\beta \]
		Result for this case follows since $\beta$ and $\beta'$ can be arbitrarily small. 
		
		Let's now suppose that there exists some $d \le \overline{d}$ such that $\alpha(\emptyset,l,d;\Pi^{n}_{1}) = 1$. Let $d_{min}$ be the smallest $d$ such that  $\alpha(\emptyset,l,d_{min};\Pi^{n}_{1})=1$ and $\alpha(\emptyset,l,d;\Pi^{n}_{1})=0$ for all $d < d_{min}$. 
		\[
		\sum_{d \le \overline{d},t} \gamma_{t}p_{d}^{t}\alpha(\emptyset,t,d;\Pi_{1}^{n}) \le \sum_{d < d_{min},t}\gamma_{t}p_{d}^{h}\alpha(\emptyset,t,d;\Pi_{1}^{n}) + \alpha(\emptyset,l,d_{min};\Pi_{1}^{n})\sum_{d_{min} \le d \le \overline{d},t}\gamma_{t}p_{d}^{h}
		\] 
		From properties of $\mathcal{A}^{s}_{n}(\beta,\overline{d})$, we know that $\frac{N_{t,d_{1},s}(g^{n},z)}{N_{t,d_{1}}} - \frac{N_{t,d_{2},s}(g^{n},z)}{N_{t,d_{2}}} \le 2\beta$ for all $d_{2} \ge d_{1}$. Define $\alpha^{max}(s,t)$ to be $max\{ \alpha(s,t,d|\Pi_{1}^{n}) \}_{d_{min} \le d \le \overline{d} } $. We then have the following properties of receivers' actions upon observing different signals:
		\begin{enumerate}
			\item $\alpha^{max}(s,t) \ge  \alpha(s,t,d|\Pi_{1}^{n} )$ for all $s \in S$, $t \in \{h,l\}$ and $ d_{min} \le d \le \overline{d} $
			\item $\alpha(\emptyset,l,d_{min}|\Pi_{1}^{n} ) \ge \alpha(\emptyset,t,d|\Pi_{1}^{n} )$ for all $d$ and $t$.
			\item $\alpha(\emptyset,l,d|\Pi_{1}^{n} ) =0$ for all $d < d_{min}$. 
		\end{enumerate} 
		From these, we have that for all $s$
		\begin{multline}
			\sum_{t,d \le \overline{d} }p_{d}^{t}\gamma_{t}
			\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\alpha(s,t,d;\Pi^{n}_{1}) +  p_{d}^{t}\gamma_{t}(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\alpha(\emptyset,t,d;\Pi^{n}_{1}) \le  \\
			4\beta + \sum_{t,d < d_{min} }p_{d}^{h}\gamma_{t}
			\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}}\alpha(s,t,d;\Pi^{n}_{1}) +  p_{d}^{h}\gamma_{t}(1-\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}})\alpha(\emptyset,t,d;\Pi^{n}_{1}) + \\
			\sum_{t}\gamma_{t} \alpha^{max}(s,t)\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}\sum_{d_{min} \le d \le \overline{d} }p_{d}^{h}
			+ \sum_{t}\gamma_{t} \alpha(\emptyset,t,d_{min};\Pi^{n}_{1})(1-\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}) \sum_{d_{min} \le d \le \overline{d} }p_{d}^{h}
		\end{multline}
		Therefore, in this case, \ref{exprop3eq1} is smaller than 
		\begin{multline} \label{exprop3eq4}
			\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi_{1}(s|\omega) \\
			\bigg[  (1-b_{1}(\omega)) v\big(2\beta+\sum_{d < d_{min},t}\gamma_{t}p_{d}^{h}\alpha(\emptyset,t,d;\Pi_{1}^{n}) + \alpha(\emptyset,l,d_{min};\Pi_{1}^{n})\sum_{d_{min} \le d \le \overline{d},t}\gamma_{t}p_{d}^{h}\big) +\\
			b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}_{1}) \\
			v\big(6\beta+ \sum_{t,d < d_{min} }p_{d}^{h}\gamma_{t}
			\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}}\alpha(s,t,d;\Pi^{n}_{1}) +  p_{d}^{h}\gamma_{t}(1-\frac{N_{t,d,s}(g^{n},z)}{N_{t,d}})\alpha(\emptyset,t,d;\Pi^{n}_{1}) + \\
			\sum_{t}\gamma_{t} \alpha^{max}(s,t)\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}\sum_{d_{min} \le d \le \overline{d} }p_{d}^{h}
			+ \sum_{t}\gamma_{t} \alpha(\emptyset,t,d_{min};\Pi^{n}_{1})(1-\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}) \sum_{d_{min} \le d \le \overline{d} }p_{d}^{h}   \big) 
			\bigg]  
			+ \beta v(1)
		\end{multline}
		By convexity and definition of $\beta$, \ref{exprop3eq4} is smaller than 
		\begin{multline} \label{prop3eq55}
			\beta  v(1) + \beta'+	\sum_{d < d_{min} }p_{d}^{h}\hat{V}^{ext}(d,\Pi_{1}^{n}) + 	\sum_{d_{min} \le d \le \overline{d}} p_{d}^{h} \sum_{\omega} \mu_{s}(\omega) \\
			\bigg[  \bigg(1-b_{1}(\omega) + b_{1}(\omega)\sum_{s \in S} \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})(1-\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}})  \bigg)v(1)  + \\
			b_{1}(\omega) \sum_{s \in S} \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}v\big(\sum_{t}\gamma_{t}\alpha^{max}(s,t) \big)\bigg]
		\end{multline}
		It's  sufficient for us to show that the fourth term in \ref{prop3eq55} is smaller than $\sum_{d_{min} \le d \le \overline{d}} p_{d}^{h}V_{pub}^{*}$. Define those signals with $\alpha^{max}(s,l)=1 $ as $S_{good}$, those with $\alpha^{max}(s,l)=0$ but $\alpha^{max}(s,h)=1$ as $S_{int}$ and the rest as $S_{bad}$. Consider the public signal strategy $(\pi_{3},b_{3}$ defined as follows:
		\[
		b_{3}(\omega) = b_{1}(\omega)\sum_{s \in S} \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
		}
		\]
		For $j \in \{good,int,bad\}$ and $\omega=1$
		\[
		\pi_{3}(s_{j}|\omega=1) = 
		\frac{b_{1}(\omega=1)\sum_{s \in S_{j}} \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
		}}{b_{2}(\omega=1)}
		\]
		For $s_{int}$, set 
		\begin{multline}
			\pi_{3}(s_{int}|\omega=0 ) =min\{ \frac{b_{3}(\omega=1)\pi_{3}(s_{int}|\omega=1) \mu_{h}(\omega=1) }{ b_{3}(\omega=0) \mu_{h}(\omega=0)  } ,  \\ \frac{b_{1}(\omega=0)\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
			}}{b_{3}(\omega=0)}    \} 
		\end{multline}
		For $s_{good}$, set 
		\begin{multline}
			\pi_{3}(s_{good}|\omega=0 ) =min \{ \frac{b_{3}(\omega=1)\pi_{3}(s_{good}|\omega=1) \mu_{l}(\omega=1) }{ b_{3}(\omega=0) \mu_{l}(\omega=0)  }, \\ 
			\frac{b_{1}(\omega=0)\sum_{s \in S_{good}} \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d,s}(g^{n},z)}{N_{l,d}
			}}{b_{2}(\omega=0)} \}
		\end{multline}
		One can verify that $\pi_{3}(s_{int}|\omega=0 ) + \pi_{3}(s_{good}|\omega=0 ) \le 1$. For $s_{bad}$, set 
		\[
		\pi_{3}(s_{bad}|\omega=0) = 1- \pi_{3}(s_{int}|\omega=0 ) - \pi_{3}(s_{good}|\omega=0 )
		\]
		By construction, all receivers choose action 1 upon observing signal $s_{good}$ with the public signal structure $(\pi_{3},b_{3})$. Similarly, type $h$ receivers choose action 1 upon observing $s_{int}$.
		
		Also, receivers observe $\emptyset$ in each state with the same probability as that of a receiver with type $l$ and degree $d_{min}$ under network signal structure $\Pi^{n}_{1}$. Therefore, all receivers must choose action 1 upon observing $\emptyset$. 
		
		For each $s \in S_{int}$, there must exist some $d$ between $d_{min}$ and $\overline{d}$ such that 
		\begin{multline}
			\mu_{h}(\omega=1) b_{1}(\omega=1) \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
		}    \ge \\
		 \mu_{h}(\omega=0) b_{1}(\omega=0) \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{h,d,s}(g^{n},z)}{N_{h,d}
	}
		\end{multline}
		If $\hat{\zeta}^{s}(h,d) \ne 0$, using similar steps as in proof of lemma \ref{lemmavhatexten}, this inequality implies that 
		\begin{multline}
			2(1 + \frac{\hat{\zeta}^{s}(l,d_{min})}{\hat{\zeta}^{s}(h,d)})\beta+ \mu_{h}(\omega=1) b_{1}(\omega=1) \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
		} \ge \\  - 2(1 + \frac{\hat{\zeta}^{s}(l,d_{min})}{\hat{\zeta}^{s}(h,d)})\beta + \mu_{h}(\omega=0) b_{1}(\omega=0) \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
	}
		\end{multline}
		Therefore
		\begin{multline}
			\mu_{h}(\omega=1) b_{1}(\omega=1) \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
			} \ge  \\   - 4(1 + \frac{\hat{\zeta}^{s}(l,d_{min})}{\hat{\zeta}^{s}(h,d)} )\beta + \mu_{h}(\omega=0) b_{1}(\omega=0) \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
			}
		\end{multline}
		Let $K_{4}$ denote the largest value of $\frac{\hat{\zeta}^{s}(l,d_{min})}{\hat{\zeta}^{s}(h,d)}$ over all $s \in S_{int}$ and $d \le \overline{d}$ with $\hat{\zeta}^{s}(h,d)$.
		Summing over $s \in S_{int}$, we have by definition
		\begin{multline}
			\pi_{3}(s_{int}|\omega=0)b_{3}(\omega=0) \ge   \\ b_{1}(\omega=0)\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
			} - \frac{4|S|(2 + K_{4} )\beta}{\mu_{h}(\omega=0)}
		\end{multline}
		For each $s \in S_{good}$, there must exist some $d'$ between $d_{min}$ and $\overline{d}$ such that 
		\begin{multline}
			\mu_{l}(\omega=1) b_{1}(\omega=1) \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{l,d',s}(g^{n},z)}{N_{l,d'}
		}\ge \\
		 \mu_{l}(\omega=0) b_{1}(\omega=0) \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d',s}(g^{n},z)}{N_{l,d'}
	}
		\end{multline}
		If $\hat{\zeta}^{s}(l,d') \ne 0$, using similar steps as in proof of lemma \ref{lemmavhatexten}, this inequality implies that 
		\begin{multline}
		2(1 + \frac{\hat{\zeta}(l,d_{min})}{\hat{\zeta}(l,d')})\beta+ \mu_{l}(\omega=1) b_{1}(\omega=1) \pi_{1}(s|\omega=1)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=1;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
		} \\
	\ge  - 2(1 + \frac{\hat{\zeta}(l,d_{min})}{\hat{\zeta}(l,d')})\beta + \mu_{l}(\omega=0) b_{1}(\omega=0) \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
	}
		\end{multline}
		Let $K_{5}$ denote the largest value of $\frac{\hat{\zeta}^{s}(l,d_{min})}{\hat{\zeta}^{s}(l,d)}$ over all $s \in S_{good}$ and $d \le \overline{d}$ with $\hat{\zeta}^{s}(l,d)$.
		Summing over $s \in S_{good}$, we have by definition
		\begin{multline}
			\pi_{3}(s_{good}|\omega=0)b_{3}(\omega=0) \ge   \\ b_{1}(\omega=0)\sum_{s \in S_{good}} \pi_{1}(s|\omega=0)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n},\omega=0;\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}
			} -\frac{4|S|(2 + K_{5}   )\beta}{\mu_{l}(\omega=0)}
		\end{multline}
		
		Combining these facts, sender's payoff using $(\pi_{3},b_{3})$ is at least
		\begin{multline} \label{expropeq12}	
			\sum_{\omega} \mu_{s}(\omega)\bigg[
			\bigg( 1-b_{1}(\omega)  + b_{1}(\omega)\sum_{s \in S} \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})(1-\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}})                          \bigg)v\big(1\big) \\
			+b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}v(1)      \\
			+b_{1}(\omega) \sum_{s \in S_{int}}                 \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1})\frac{N_{l,d_{min},s}(g^{n},z)}{N_{l,d_{min}}}v(\gamma_{h})            
			\bigg]  \\  -\frac{4|S|(2 + K_{5}   )\beta}{\mu_{l}(\omega=0)}v(1)- \frac{4|S|(2 + K_{4} )\beta}{\mu_{h}(\omega=0)}v(1)
		\end{multline}	
		The result then follows since $\beta'$ and $\beta$ can be arbitrarily small and $v(1)$ is bounded. 

		\subsection{Existence of limit}
I show that for $n$ large enough, sender's payoff can be arbitrarily close to the limsup of $V_{net}^{*}(D^{(n)})$. To do that I first prove a useful lemma, 
\begin{lemma} \label{lemmanobadsignal}
	For any $\beta'>0$, there exists some $n_{1}$ such that for all games with $n \ge n_{1}$, if some sender's strategy achieves some payoff $V$ for the sender, then there exists another strategy $\Pi_{2}^{n}$ that achieves at least $V-\beta'$ and
	satisfies \begin{enumerate}
		\item There exists no signal that convinces neither type of receivers. 
		\item For all $s \in S_{good}$, it must be the case that $\pi_{3}(s|\omega=1)b(\omega=1)\mu_{l}(\omega=1) = \pi_{3}(s|\omega=0)b(\omega=0)\mu_{l}(\omega=0)$.
	\end{enumerate} 
\end{lemma}
\begin{proof}
	For any $\beta'>0$, we can find a $\hat{\beta }>0$ such that $sup( v(x+8\hat{\beta})-v(x)) < \beta'$. For this $\hat{\beta}$, we can find some $\overline{d}$ such that $\sum_{d>\overline{d}} (\gamma_{h}p_{d}^{h}+\gamma_{l}p_{d}^{l}	) < \hat{\beta} $. Fix this $\overline{d}$. We can find some $\beta < \hat{\beta}$ such that $4\beta + \frac{4\beta \zeta(t,d)}{\zeta(l,1)} \le \zeta(t,d) - \hat{\zeta}(t,d)$ for all $t$ and $d \le \overline{d}$, and $\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{1- 2 \beta \frac{\mu_{h}(\omega=1)}{\mu_{h}(\omega=0)}}{1- 2 \beta } < 1$.
	By lemmas proved before and assumption 1 on $D$, we can find some $n_{1}$ such that for all $n>n_{1}$, the following conditions are satisfied:
	\begin{enumerate}
		\item $\sum_{d > \overline{d}}  \frac{N_{h,d}+N_{l,d}}{n}  < \hat{ \beta }  $
		\item $\frac{N_{t,d}}{n}  \in [\gamma_{t}p_{d}(1-\beta) ,  \gamma_{t}p_{d} (1+ \beta)]  $ for $t\in \{h,l\}$ and all $d \le \overline{d}$. 
		\item $Pr(g^{n} \in \mathcal{A}_{n}(\beta,\overline{d} )  ) > 1-\beta$
	\end{enumerate}
	
	Let $\Pi_{1}^{n}$ achieve payoff $V$. If the conditions stated in lemma are satisfied by $\Pi_{1}^{n}$. We are done. Suppose this is not the case.
	
	In the game with $n$ receivers, sender's payoff from $\Pi^{n}_{1}$ is
	
	\begin{multline} \label{sec6eq1}
		\sum_{\omega} \mu_{s}(\omega) \sum_{s \in S} \pi_{1}(s|\omega)\bigg[  (1-b_{1}(\omega)) v(\sum_{t,d}\frac{N_{t,d}}{n} \alpha(\emptyset,t,d;\Pi^{n}_{1})) +\\
		b_{1}(\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1}) v(\sum_{t,d}\frac{N_{t,d,s}(g^{n},z)}{n}\alpha(s,t,d;\Pi^{n}_{1}) +  (1-\frac{N_{t,d,s}(g^{n},z)}{n})\alpha(\emptyset,t,d;\Pi^{n}_{1})  )    
		\bigg]
	\end{multline}
	Using steps essentially the same in proof of proposition 1 (and 3) above, \ref{sec6eq1} is smaller than
	\begin{multline} \label{sec6eq3}
		\beta  v(1) + \beta'+ \sum_{\omega}\mu_{s}(\omega) \big[ (1-b(\omega))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		\sum_{s \in S_{good}}b_{1}(\omega) \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1}) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		C_{1}(z,g^{n})\zeta(t,d) +  p_{d}\gamma_{t}(1-C_{1}(z,g^{n})\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		\sum_{s \in S_{int}}b_{1}(\omega)\pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1}) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{C}_{1}(z,g^{n})\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{C}_{1}(z,g^{n})\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		\sum_{s \in S_{bad}}b_{1}(\omega) \pi_{1}(s|\omega)\sum_{g^{n},z}Pr(g^{n})Pr(z|s,g^{n};\Pi^{n}_{1}) 
		v\big( \sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1}) \big)
		\big]  
	\end{multline}
	By definition of $C_{1}$ and $\hat{C}_{1}$, we can rewrite this as
	\begin{multline} \label{sec6eq5}
		\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
		\big]  +\beta  v(1) +\beta'
	\end{multline}
	Going through essentially the same steps, we can also show that it's bounded below by
	\begin{multline} \label{sec6eq4}
		\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
		\big]  -\beta' -\beta  v(1)
	\end{multline}
	
	I first show that we can find some $\Pi_{2}^{n}$ such that $Pr(z \in L_{1}|s) >  \frac{\beta}{\zeta(l,1) - \beta }  $ for all $S_{good}$. If this is the case for $\Pi_{1}^{n}$, we are done. Suppose not and let $S_{good}'$ denote the set of signals in $S_{good}$ such that $Pr(z \in L_{1}|s) > \frac{\beta}{\zeta(l,1) - \beta }$. In this case, sender's payoff is bounded above by 
	\begin{multline} 
		\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
		\big]    + \frac{\beta}{\zeta(l,1) - \beta }v(1) +\beta v(1) +\beta'
	\end{multline}
	Consider sender's strategy $\Pi_{2}^{n}$ defined as follows 
	\[
	b_{2}(\omega)\pi_{2}(s|\omega) = b_{2}(\omega)\pi_{2}(s|\omega) \text{ for all }s \notin S_{good} / S_{good}' \qquad b_{2}(\omega) = \sum_{s \notin S_{good} / S_{good}'} b_{2}(\omega)\pi_{2}(s|\omega)
	\]
	Let the seeding strategy for each signal be the same as in $\Pi_{1}^{n}$
	One can check that by construction receivers' action upon each observation is the same as when they face $\Pi_{1}^{n}$. Therefore, sender's payoff is bounded below by 
	\begin{multline} 
		\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
		\big]   -\beta  v(1) - \beta'
	\end{multline}
	Let's denote elements in $S_{good}'$ by $\{s_{1}',s_{2}',...\}$ and denote $1-\sum_{s \in S_{good}' \cup S_{int} } b_{2}(\omega=0)\pi_{2}(s | \omega=0)$ by $K$. 
	Now, we construct $\Pi_{3}^{n}$ from $\Pi_{2}^{n}$ using the following procedure: 
	Starting from $j=1$,
	\begin{enumerate}
		\item Let $b_{3}(\omega=0)\pi_{3}(s_{j}'|\omega=0) = \frac{b_{2}(\omega=1)\pi_{2}(s_{j}'|\omega=1) \mu_{l}(\omega=1) }{\mu_{l}(\omega=0)  }$ if 
		\begin{multline}
			\frac{b_{2}(\omega=1)\pi_{2}(s_{j}'|\omega=1) \mu_{l}(\omega=1) }{\mu_{l}(\omega=0)  } - b_{2}(\omega=0)\pi_{2}(s_{j}'|\omega=0) \\ \le K -\sum_{i=1}^{j-1}  ( b_{3}(\omega=0)\pi_{3}(s_{i}'|\omega=0) - b_{2}(\omega=0)\pi_{2}(s_{i}'|\omega=0)   )
		\end{multline}
		\item Otherwise, set 
		\[
		b_{3}(\omega=0)\pi_{3}(s_{j}'|\omega=0)	=	b_{2}(\omega=0)\pi_{2}(s_{j}'|\omega=0) + K -\sum_{i=1}^{j-1}  ( b_{3}(\omega=0)\pi_{3}(s_{i}'|\omega=0) - b_{2}(\omega=0)\pi_{2}(s_{i}'|\omega=0))
		\]
	\end{enumerate}
	Set $\pi_{3}(s|\omega=1)b_{3}(\omega=1) = \pi_{2}(s|\omega=1)b_{2}(\omega=1)$ for all $s \in S_{good}$.
	Set $\pi_{3}(s|\omega)b_{3}(\omega) = \pi_{2}(s|\omega)b_{2}(\omega)$ for all $s \in S_{int}$ and let $b_{3}(\omega) =  \sum_{s \in S_{good}' \cup S_{int}} \pi_{3}(s|\omega)b_{3}(\omega)$. Again, let seeding strategies remain the same. 
	
	One can easily verify that by construction $b(\omega)\le 1$, and receivers choose action 1 upon observing signals in $S_{good}'$ and type $h$ receivers choose action 1 upon observing signals in $S_{int}$. Also, since we are not changing the probabilities in state $\omega=1$, the probability that receivers observe $\emptyset$ in state $\omega=1$ is unchanged. In state $\omega=0$, we increased the probabilities that signals in $S_{good}'$ are realised and visible by $K$, and this decreases the probability of observing $\emptyset$ in state $\omega$ by at least $K \beta$. The probabilities of signals in $S_{int}$ being realised and visible are unchanged in state $\omega=0$. We reduced the probability of signals in $S_{bad}$ being realised and visible with probability by at most $K$, and this increases the probability of observing $\emptyset$ by at most $\beta K$. Therefore, compared to $\Pi_{2}^{n}$, receivers must observe $\emptyset$ in state 0 with weakly lower probability and thus must have weakly higher priors upon observing $\emptyset$. We also know that 
	\[
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) \ge v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big)
	\]
	Therefore, sender's payoff from $\Pi_{3}^{n}$ is bounded below by 
	\begin{multline} \label{equation75}
		\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
		b_{1}(\omega) \sum_{s \in S_{good}'} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
		b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
		v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
		\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
		\big]   -\beta v(1) - \beta'
	\end{multline}
$\Pi_{3}^{n}$ will surely satisfy condition 1 in the lemma. If it also satisfies condition 2 in the lemma, the proof is finished. Suppose not, then by how $\Pi_{3}^{n}$ is constructed, we must have $b_{3}(\omega=0)=1$.  

	Now suppose that $Pr(z \in L_{1}|s) \ge 1- 4\beta/\zeta(h,1)$ for all $s \in S_{good}'$. Therefore conditional on $s \in S_{good}$ being realised, the probability that a receiver with type $t$ and degree $d \le \overline{d}$ observes it with probability at least
	\[
	Pr(z \in L_{1}|s)\zeta(t,d) -2\beta \ge \zeta(t,d) -2\beta - 4\beta\frac{\zeta(t,d)}{\zeta(h,1)}
	\]
	Similarly, conditional on some $s \in S_{int}$ being realised, the probability that a receiver with type $t$ and degree $d \le \overline{d}$ observes it with probability at most
	\[
	\hat{\zeta}(t,d) + 2 \beta
	\]
	Construct $\Pi_{5}^{n}$ from $\Pi_{3}^{n}$ in the following way. First, for all $s \in S_{good}'$, let
	\[
	b_{5}(\omega=1)\pi_{5}(s|\omega=1) = b_{3}(\omega=1)\pi_{3}(s|\omega=1)   \qquad  b_{5}(\omega=0)\pi_{5}(s|\omega=0) =\frac{b_{5}(\omega=1)\pi_{5}(s|\omega=1) \mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}
	\]
	Let $K_{2} =  \sum_{s \in S_{good}'} b_{5}(\omega=0)\pi_{5}(s|\omega=0) - b_{3}(\omega=0)\pi_{3}(s|\omega=0)$. 
	Denote the elements in $S_{int}$ by $(s_{1}^{int},s_{2}^{int},...)$. Then, use the following procedure, starting from $i=1$
	\begin{enumerate}
		\item Let $\pi_{5}(s_{i}^{int}|\omega)$ be 0 if $K_{2}-\sum_{j=1}^{i} b_{3}(\omega=0)\pi_{3}(s_{j}^{int}|\omega=0) \ge 0$
		\item If $K_{2}-\sum_{j=1}^{i} b_{3}(\omega=0)\pi_{3}(s_{j}^{int}|\omega=0) < 0$, if the following ratio
		\[
	\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}	\frac{b_{3}(\omega=1)\pi_{3}(s_{i}^{int}|\omega=1)}{b_{3}(\omega=0)\pi_{3}(s_{i}^{int}|\omega=0) - (K-\sum_{j=1}^{i-1} b_{3}(\omega=0)\pi_{3}(s_{j}^{int}|\omega=0))}	
		\]
		is larger than 1, then set $\pi_{5}(s_{i}^{int}|\omega)=0$. Otherwise, set $b_{5}(\omega=1)\pi_{5}(s_{i}^{int}|\omega=1)=b_{3}(\omega=1)\pi_{3}(s_{i}^{int}|\omega=1)$ and $b_{5}(\omega=0)\pi_{5}(s_{i}^{int}|\omega=0)$ to be 
		\[
		b_{3}(\omega=0)\pi_{3}(s_{i}^{int}|\omega=0) - (K-\sum_{j=1}^{i-1} b_{3}(\omega=0)\pi_{3}(s_{j}^{int}|\omega=0))
		\]
		\item If $K-\sum_{j=1}^{i} b_{3}(\omega=0)\pi_{3}(s_{j}^{int}|\omega=0) > 0$ and $i < |S_{int}|$, continue steps above for $i+1$. Otherwise, terminate the process. Let $i_{end}$ be the index where the process is terminated.
	\end{enumerate}
	 For all $i > i_{end}$, let $b_{5}(\omega)\pi_{5}(s_{i}^{int}|\omega)=b_{3}(\omega)\pi_{3}(s_{i}^{int}|\omega)$. Let $b_{5}(\omega) = \sum_{s \in S_{int} \cup S_{good}'} \pi_{5}(s|\omega)b(\omega)$. Let seeding strategy be unchanged from before. 
	One can verify that $b_{5}(\omega)\le 1$. Again, by construction, all receivers choose action 1 upon observing signals in $S_{good}'$ and type $h$ receivers choose action 1 upon observing signals in $S_{int}$.
	
	I now argue that type $l$ receivers' action must be weakly higher under $\Pi_{5}$ compared to $\Pi_{3}$. Compared to $\Pi_{3}^{n}$, the probabilities of observing $\emptyset$ changed due to the following changes
	\begin{enumerate}
		\item In state 0, probability of observing signals in $S_{good}'$ increased by $K_{2}$, and probability of observing signals in $S_{int}$ decreased by $K_{2}$. Due to these changes, the probability of observing $\emptyset$ in state 0 is decreased by $(\zeta(t,d) -4 \beta- 4\beta \frac{\zeta(t,d)}{\zeta(h,1)} -\hat{\zeta}(t,d))K_{2} >0$ for receiver with degree $d$ and type $t$.
		\item Probability of observing $\emptyset$ in state 1 decreases due to decreases in probabilities of observing signals $s_{i}^{int}$ with $i < i_{end}$
		\item We know that likelihood ratio upon observing $\emptyset$ under $\Pi_{5}^{n}$ must be higher than that under $\Pi_{3}^{n}$ after these changes.
		\item Finally, we may need to decrease the probability of observing $s_{i_{end}}^{int}$. If it is decreased, then we know that the probability of observing it in state 1 is decreased by $b_{3}(\omega=1)\pi_{3}(s_{i_{end}}^{int})E(N_{s_{i_{end}}^{int},t,d}/N_{t,d} |s_{i_{end}}^{int}) $, and that in state 0 is decreased by some probability smaller than $\frac{b_{3}(\omega=1)\pi_{3}(s_{i_{end}}^{int}) \mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}E(N_{s_{i_{end}}^{int},t,d}/N_{t,d} |s_{i_{end}}^{int}) $. Therefore, after being multiplied by type $l$ receiver's prior for their respective states, probability of observing $\emptyset$ decreases more in state 1 than in state 0. This implies that if likelihood ratio of observing $\emptyset$ is higher than 1 before the change, it must also be higher than 1 after the change. 
	\end{enumerate}
	Also, since $\Pi_{3}^{n}$ has $b_{3}(\omega=1)$ and all signals used must convince type $h$ receivers, one can verify that all receivers with type $h$ must choose action 1 upon observing $\emptyset$. Therefore, payoff from $\Pi_{5}^{n}$ must also be weakly higher than that from $\Pi_{3}^{n}$, and thus bounded be low by \ref{equation75} again. 
	
	Next suppose that  $Pr(z \in L_{1}|s) < 1- \frac{4\beta }{\zeta(h,1)}$ for some $s \in S_{good}'$. Denote that set by $S_{good}''$
	From $\Pi_{3}^{n}$, we can construct the following strategy $\Pi_{4}^{n}$
	\[
	\pi_{4}(s|\omega)b_{4}(\omega) = \pi_{3}(s|\omega)b_{3}(\omega) \text{ for all }s \in S_{int} \cup (S_{good}'/S_{good}'')
	\]
	Also let the seeding strategies be the same for these signals in $S_{int}$.
	Then, let $\pi_{4}(s_{good}|\omega = 1)b_{4}(\omega=1)$ be
	\[
	\frac{\zeta(l,d=1)}{\zeta(l,d=1) +2 \beta }  b(\omega=1)\sum_{s \in S_{good}''} \pi_{3}(s|\omega=1)Pr(z \in L_{1}|s) -        \frac{2\beta }{(\zeta(l,d=1) +2 \beta) }
	\]
	\[ \pi_{4}(s_{good}|\omega = 0)b_{4}(\omega=0) = \min\{ \frac{\pi_{4}(s_{good}|\omega = 1)b_{4}(\omega=1) \mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} , 1- \sum_{s \in S_{int} \cup (S_{good}'/S_{good}'') }\pi_{4}(s|\omega=0)b_{4}(\omega=0) \}
	\]
	Let seed always hit $L_{1}$ for signal $s_{good}$. 
	Let $b_{4}(\omega) = \sum_{s \in S} \pi_{4}(s|\omega)b_{4}(\omega)$. By construction, all receivers choose action 1 upon observing $s_{good}$ and type $h$ receivers choose action 1 upon observing anything in $S_{int}$. I now argue that $\alpha(\emptyset,l,d;\Pi_{4}^{n}) \ge \alpha(\emptyset,l,d;\Pi_{3}^{n})$ for all $d \le \overline{d}$. First, suppose that 
	\[
	\pi_{4}(s_{good}|\omega =0)b_{4}(\omega=0) =  1- \sum_{s \in S_{int}\cup (S_{good}'/S_{good}'') }\pi_{4}(s|\omega =0)b_{4}(\omega=0) = \sum_{s \in S_{good}''}\pi_{3}(s|\omega=0)b_{3}(\omega=0)
	\]
	In this case, receivers with type $l$ and degree $d \le \overline{d}$ observe $s_{good}$ in state 0 with probability at least
	\[
	 \sum_{s \in S_{good}''}\pi_{3}(s|\omega=0)b_{3}(\omega=0) (\zeta(l,d)- 2 \beta)
	\]
	Under $\Pi_{3}^{n}$, the probability that receivers observe any signal in $S_{good}''$ is at most
	\[
	\sum_{s \in S_{good}''}\pi_{3}(s|\omega=0)b_{3}(\omega=0)(Pr(z \in L_{1}|s)\zeta(l,d) +2* \beta ) \le  \sum_{s \in S_{good}''}\pi_{3}(s|\omega=0)b_{3}(\omega=0) (\zeta(l,d)- 2\beta)
	\]
	The probabilities of observing other signals in state 0 is the same for $\Pi_{3}^{n}$ and $\Pi_{5}^{n}$. Therefore, the probability of observing $\emptyset$ in state 0 is weakly lower under $\Pi_{5}^{n}$ than under $\Pi_{3}^{n}$. 
	
	
	
	Receivers with type $l$ and degree $ d \le \overline{d}$ observe $s_{good}$ in state 1 with probability at most
	\[
	\zeta(l,d) b_{3}(\omega=1)\sum_{s \in S_{good}''} \pi_{3}(s|\omega=1)Pr(z \in L_{1}|s) -  2 \beta
	\]
	which is also the least probability that receivers with type $l$ and degree $d$ observe any signal in $S_{good}''$ under $\Pi_{3}^{n}$. Again, probabilities of observing any other strategies are unchanged. Therefore, the posterior upon observing $\emptyset$ must weakly increase for all receivers with type $l$ and degree $d \le \overline{d}$. 
	
	Now consider the second case with $\pi_{4}(s_{good}|\omega = 0)b_{4}(\omega=0) = \frac{\pi_{4}(s_{good}|\omega = 1)b_{4}(\omega=1) \mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}$. For type $l$ receivers with degree $d \le \overline{d}$ who have $\alpha(\emptyset,l,d,\Pi_{3}^{n})=1$, it must be the case that their posterior upon not observing signals in $S_{int} \cup (S_{good}' / S_{good}'')$ is higher than 0.5. Note that probabilities that receivers observe signals in $S_{int} \cup (S_{good}' / S_{good}'')$ are the same for $\Pi_{3}^{n}$ and $\Pi_{4}^{n}$. Therefore, these receivers must also have posterior higher than 0.5 when they don't observe signals in $S_{int} \cup (S_{good}'/ S_{good}'')$. Now, since these receivers will observe $s_{good}$ or $\emptyset$ under $\Pi_{4}^{n}$, and their posterior upon observing $s_{good}$ is exactly 0.5 by construction, we know that posterior upon observing $\emptyset$ must also be higher than 0.5. 
	
	Therefore, receivers' actions upon observing $\emptyset$ is weakly higher under $\Pi_{4}^{n}$ than under $\Pi_{3}^{n}$. This implies that sender's payoff from $\Pi_{4}^{n}$ is at least expression \ref{equation75} minus
	\[
	(1-   \frac{\zeta(l,d=1)}{\zeta(l,d=1) +2 \beta } +\frac{2\beta }{\zeta(l,d=1) +2 \beta})(1+\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)})v(1)
	\]
	Note that $\Pi_{4}$ is a strategy such that $Pr(z \in L_{1}|s) \ge 1- \frac{4 \beta }{\zeta(h,1)}$ for all signal $s$ that convince both types. Therefore, we can construct another strategy that achieves at least the same lower bound as $\Pi_{4}^{n}$, in the same way we constructed $\Pi_{5}^{n}$ for $\Pi_{3}^{n}$. 
	
	The proof is concluded since $\beta$ and $\beta'$ can be arbitrarily small and $v(1)$ is bounded. 
\end{proof}
I can show that under the following condition, $\lim_{n \rightarrow \infty} V_{net}^{*}(D^{(n)})$ exists. \\
\textbf{Condition A1}:
There exists no $d$ such that 
\[
\frac{\mu_{l}(\omega=1)}{ \mu_{h}(\omega=0) }\frac{ 1-\hat{\zeta}(l,d)\frac{\mu_{h}(\omega=0) }{\mu_{h}(\omega=1)}   }{ 1-\hat{\zeta}(l,d)  } =1
\]

From now on, suppose that condition A1 holds. 
For any  $\beta'>0$, we can find a $\hat{\beta}>0$ such that $sup( v(x+8\hat{\beta})-v(x)) < \beta'$. We can also find a $\beta < \hat{\beta}$, such that 
\[
\frac{\mu_{l}(\omega=1)}{ \mu_{h}(\omega=0) }\frac{ 1-(\hat{\zeta}(l,d) - 2\beta)\frac{\mu_{h}(\omega=0) }{\mu_{h}(\omega=1)}   }{ 1-(\hat{\zeta}(l,d) - 2\beta)} \ge 1
\]  
if
\[
\frac{\mu_{l}(\omega=1)}{ \mu_{h}(\omega=0) }\frac{ 1-\hat{\zeta}(l,d)\frac{\mu_{h}(\omega=0) }{\mu_{h}(\omega=1)}   }{ 1-\hat{\zeta}(l,d)  } \ge 1
\] and $\beta$ also satisfies 
\[
\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{ 1- \frac{\mu_{h}(\omega=0) }{ \mu_{h}(\omega=1)} 2 \beta}{1-   + 2 \beta } < 1
\]
For this $\beta$, we can find some $\overline{d}$ such that $\sum_{d>\overline{d}} (\gamma_{h}p_{d}^{h}+\gamma_{l}p_{d}^{l}	) <\beta $. Fix this $\overline{d}$. By lemmas above and construction, we can find some $n_{1}$ such that for all $n>n_{1}$, the following conditions are satisfied:
\begin{enumerate}
	\item $\sum_{d > \overline{d}}  \frac{N_{h,d}+N_{l,d}}{n}  < \beta  $
	\item $\frac{N_{t,d}}{n}  \in [\gamma_{t}p_{d}(1-\beta) ,  \gamma_{t}p_{d} (1+ \beta)]  $ for $t\in \{h,l\}$ and all $d \le \overline{d}$. 
	\item $Pr(g^{n} \in \mathcal{A}_{n}(\beta,\overline{d} )  ) > 1-\beta$
	\item If there's some strategy $\Pi_{1}^{n}$ that achieves payoff $V$, then there exists another strategy $\Pi_{2}^{n}$ that achieves at least $V-\beta$ and satisfies conditions stated in lemma \ref{lemmanobadsignal}.
\end{enumerate}

By definition and point 4 above, we know that we can find some $n \ge n_{1}$ and some strategy $\Pi_{1}^{n}$ that achieves payoff at least $limsup_{n} V^{*}_{net}(D^{n}) -2\beta $, and it satisfies the conditions in lemma \ref{lemmanobadsignal}. Let $S_{good}$ denote the set of signals that convince both types of receivers, $S_{int}$ denote the set of signals that convince only type $h$ receivers. 

Also, let $N_{t,d,s}(g^{n},z)$ denote the number of type $t$ degree $d$ receivers that observe signal $s$, given network $g^{n}$, seeds $z$ and signal $s$ being realised and visible. 
In the game with $n$ receivers, sender's payoff from $\Pi^{n}_{1}$ is given by
Following the same steps in proof of lemma \ref{lemmanobadsignal}, sender's payoff from $\Pi^{n}_{1}$ is bounded above by \ref{sec6eq5}, reproduced below.
\begin{multline}
	\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big]  +\beta v(1) +\beta'
\end{multline}
Similarly, given any strategy $\Pi^{n}$ that satisfies conditions in \ref{lemmanobadsignal}, sender's payoff is bounded below by \ref{sec6eq4}
\begin{multline} 
	\sum_{\omega}\mu_{s}(\omega) \big[ (1-b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)Pr(z \in L_{1}|s )  - 	b(\omega)\sum_{s \in S_{int}}\pi(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n})\big) +\\
b(\omega) \sum_{s \in S_{good}} \pi(s|\omega)Pr(z \in L_{1}|s ) 
v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}) \big) + \\
b(\omega)\sum_{s \in S_{int}}\pi(s|\omega)Pr(z \in \hat{L}_{1}|s)
v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}) \big) 
\big]  - \beta v(1) - \beta'
\end{multline}
We consider two cases. First, suppose that no type $l$ receivers with degree less than $\overline{d}$ chooses action 1 upon observing $\emptyset$ with strategy $\Pi_{1}^{n}$. We can find some $d_{max}$ such that type $h$ receiver with degree $d_{max}$ chooses 1 upon observing $\emptyset$ and those with degrees $d_{max}< d \le \overline{d}$ choose 0 upon observing $\emptyset$. We know that the probability that receivers with type $h$ and degree $d_{max}$ observe signals in $S_{good}$ with probability at least
\begin{equation}
 max\{0,\zeta(h,d_{max})b(\omega=1)\sum_{s \in S_{good}}\pi_{2}(s|\omega=1)Pr(z \in L_{1}|s)-2\beta\} \equiv OB_{good}
\end{equation}
 in state $\omega=1$.
Similarly, they observe signals in $S_{int}$ with probability at least in state $\omega=1$
\[
max\{0,\hat{\zeta}(h,d_{max})b(\omega=1)\sum_{s \in S_{int}}\pi_{2}(s|\omega=1)Pr(z \in \hat{L}_{1}|s) - 2\beta	\} \equiv OB_{int}
\]
Therefore, the likelihood ratio upon observing $\emptyset$ of receiver with type $h$ and degree $d_{max}$ mast satisfy
\[
\frac{\mu_{h}(\omega=1)}{\mu_{h}(\omega=0)} \frac{1-OB_{good} - OB_{int}   }{ 1-\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}OB_{good}  - min\{1-\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}OB_{good},\frac{\mu_{h}(\omega=1)}{\mu_{h}(\omega=0)}OB_{int}\}  } \ge 1
\]
For any game with $n \ge n_{2}$ players, consider the following strategy for sender
\[
b_{2}(\omega=1)\pi_{2}(s_{good}|\omega=1) = OB_{good}/(\zeta(h,d_{max})+ 2 \beta ) 
\]
\[
b_{2}(\omega=1)\pi_{2}(s_{int}|\omega=1) = OB_{int}/(\hat{\zeta}(h,d_{max})+2 \beta )
\]
\[
b_{2}(\omega=0)\pi_{2}(s_{good}|\omega=0) =  \frac{b_{2}(\omega=1)\pi_{2}(s_{good}|\omega=1) \mu_{l}(\omega=1)}{\mu_{l}(\omega=0)} 
\]
\[
b_{2}(\omega=0)\pi_{2}(s_{int}|\omega=0) =  min \{\frac{b_{2}(\omega=1)\pi_{2}(s_{int}|\omega=1) \mu_{h}(\omega=1)}{\mu_{h}(\omega=0)} , 1-b_{2}(\omega=0)\pi_{2}(s_{good}|\omega=0) \}
\]
\[
b_{2}(\omega) = b_{2}(\omega)\pi_{2}(s_{good}|\omega) + b_{2}(\omega)\pi_{2}(s_{int}|\omega)
\]
Let the seed always hit relevant giant component. 
One can verify that $b_{2}(\omega) \le 1$. If $b_{2}(\omega=0)=1$, then one can easily verify that all receivers with type $h$ must choose action 1 upon observing $\emptyset$. Otherwise, receiver with degree $d_{max}$ and type $h$ observes $s_{good}$ in state 1 with probability at most $OB_{good}$
and $s_{int}$ in state 1 with probability at most $OB_{int}$.
Therefore, likelihood ratio upon observing $\emptyset$ is at least
\[
\frac{\mu_{h}(\omega=1)}{\mu_{h}(\omega=0)} \frac{1-OB_{good} - OB_{int}   }{ 1-\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}OB_{good}  - \frac{\mu_{h}(\omega=1)}{\mu_{h}(\omega=0)}OB_{int}  } \ge 1
\]
Therefore, we know that receivers with both types choose action 1 upon observing $s_{good}$, and type $h$ receivers choose 1 upon observing $s_{int}$. Type $h$ receivers with degree weakly less than $d_{max}$ choose action 1 upon observing $\emptyset$. We can bound sender's payoff below by
\begin{multline} \label{sec6eq6}
	-\beta v(1) - \beta'+ \sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{2}(\omega)\pi_{2}(s_{good}|\omega)  - b_{2}(\omega)\pi_{2}(s_{int}|\omega))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{2}(\omega)\pi_{2}(s_{good}|\omega)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{2}(\omega)\pi_{2}(s_{int}|\omega)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big]  
\end{multline}
From how the strategies are constructed, we know that 
\[
b_{1}(\omega=1)\sum_{s \in S_{good}}\pi_{1}(s|\omega=1)Pr(z \in L_{1}|s)	- b_{2}(\omega=1)\pi_{2}(s_{good}|\omega=1)   \le 4\beta/(\zeta(h,d=1))
\]
We also know that 
\[
b_{1}(\omega=0)\sum_{s \in S_{good}}\pi_{1}(s|\omega=0)Pr(z \in L_{1}|s)	- b_{2}(\omega=0)\pi_{2}(s_{good}|\omega=0)   \le \frac{\mu_{l}(\omega=1) }{\mu_{l}(\omega=0) }4\beta/(\zeta(h,d=1))
\]
Similarly, we have
\[
b_{1}(\omega=1)\sum_{s \in S_{int}}\pi_{1}(s|\omega=1)Pr(z \in L_{1}|s)	- b_{2}(\omega=1)\pi_{2}(s_{int}|\omega=1)   \le min\{1,4\beta/(\hat{\zeta}(h,d=1))\}
\]
and
\[
b_{1}(\omega=0)\sum_{s \in S_{int}}\pi_{1}(s|\omega=0)Pr(z \in L_{1}|s)	- b_{2}(\omega=0)\pi_{2}(s_{int}|\omega=0)   \le	min\{1,\frac{\mu_{h}(\omega=1) }{\mu_{h}(\omega=0) } 4\beta/(\hat{\zeta}(h,d=1))\}
\]
Also, because we know that $ v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) \le v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big)  \le v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big)$, we know that sender's payoff from $\Pi_{2}$ is at least
\begin{multline} 
	\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big]  \\
	- \bigg(4\beta/(\zeta(h,d=1)) + \frac{\mu_{l}(\omega=1) }{\mu_{l}(\omega=0) }4\beta/(\zeta(h,d=1)) \bigg)v(1)-\beta v(1)-\beta'  \\
-min\{2,4\beta/(\hat{\zeta}(h,d=1))\bigg(1	 + \frac{\mu_{h}(\omega=1) }{\mu_{h}(\omega=0) } \bigg)\} \\ (  v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) -v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) )
\end{multline}
If $\hat{\zeta}(h,d=1) > 0$, then the result follows since $\beta$ and $\beta'$ can be arbitrarily small and $v(.)$ is bounded. If $\hat{\zeta}(h,d=1) = 0$, then we must have $\hat{\zeta}(h,d) = 0$ for all $d$, and therefore the last term of the expression above is equal to 0. The result then follows since again $\beta$ and $\beta'$ can be arbitrarily small and $v(.)$ is bounded.


Now, we consider the second case, where there exists some $d_{min} \le \overline{d}$ such that all type $l$ receivers with degree lower than $d_{min}$ choose action 0 upon observing $\emptyset$, and those with $d_{min}$ choose action 1 upon observing $\emptyset$.
Receivers with type $t$ and degree $d_{min}$ observe signals in $S_{int}$ in state 0 with probability at most
\[
b_{1}(\omega=0)\hat{\zeta}(l,d_{min}) \sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1}) + 2\beta
\]
This implies that their likelihood ratio conditional on not observing signals in $S_{int}$ (i.e. conditional on observing signals in $S_{good}$ or $\emptyset$) is at most
\[
\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{ 1- \frac{\mu_{h}(\omega=0) }{ \mu_{h}(\omega=1)}(b_{1}(\omega=0) \hat{\zeta}(l,d_{min}) \sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1} ) + 2 \beta)}{1-  (b_{1}(\omega=0)\hat{\zeta}(l,d_{min})\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1} ) + 2 \beta) } 
\]
which must be weakly greater than 1 since these receivers choose action 1 upon observing signals in $S_{good}$ or $\emptyset$. Also, this implies that $\frac{|\hat{L}_{1}|}{n}$ must not converge to 0, and thus $\hat{ \zeta }(t,d)$ must be positive 0 for all $t$ and $d$. This implies that 
\[
\frac{\mu_{l}(\omega=1)}{ \mu_{h}(\omega=0) }\frac{ 1-\hat{\zeta}(l,d_{min})\frac{\mu_{h}(\omega=0) }{\mu_{h}(\omega=1)}   }{ 1-\hat{\zeta}(l,d_{min})  } \ge 1
\]
and thus
\begin{equation} \label{equation76}
	\frac{\mu_{l}(\omega=1)}{ \mu_{h}(\omega=0) }\frac{ 1-(\hat{\zeta}(l,d_{min}) - 2\beta)\frac{\mu_{h}(\omega=0) }{\mu_{h}(\omega=1)}   }{ 1-(\hat{\zeta}(l,d_{min}) - 2\beta)} \ge 1
\end{equation}

Consider the following strategy $\Pi_{3}^{n}$ for any $n \ge n_{1}$. 
\[\pi_{3}(s_{int} |\omega=0)b_{3}(\omega=0) = min\{1, \frac{\hat{\zeta}(l,d_{min})}{\hat{\zeta}(l,d_{min})- 2\beta}b_{1}(\omega=0)\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1}) + \frac{2\beta}{ \hat{\zeta}(l,d_{min})- 2\beta}\}\]
\[
\pi_{3}(s_{good}|\omega =0)b_{3}(\omega=0) = 1 -\pi_{3}(s_{int}|\omega =0)b_{3}(\omega=0) 
\]
\[
\pi_{3}(s_{good}|\omega =1)b_{3}(\omega=1) =\frac{\mu_{l}(\omega=0)}{\mu_{l}(\omega=1)} \pi_{3}(s_{good} =0)b_{3}(\omega=0)
\]
\[
\pi_{3}(s_{int}|\omega =1)b_{3}(\omega=1)= \frac{\mu_{h}(\omega=0)}{\mu_{h}(\omega=1)}  \pi_{3}(s_{good} =0)b_{3}(\omega=0)
\]
Let $b_{3}(\omega) =\pi_{3}(s_{good}|\omega )b_{3}(\omega) +\pi_{3}(s_{int} |\omega)b_{3}(\omega)$ and one can verify that $b_{3}(\omega)\le 1$. 

If $\pi_{3}(s_{int} |\omega=0)b_{3}(\omega=0)=1$, then all receivers with degrees higher than $d_{max}$ observe $s_{int}$ in state 0 with probability at least $\hat{\zeta}(l,d_{min})-2\beta$ and thus will choose
will choose action 1 upon observing $\emptyset$ by equation \ref{equation76}. If $\pi_{3}(s_{int} |\omega=0)b_{3}(\omega=0) \ne 1$,
receivers with type $l$ and degree $d_{min}$ or higher observe $s_{int}$ in state $\omega$ with probability at least
\[
\hat{\zeta}(l,d_{min})b_{1}(\omega=0)\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1}) + 2\beta
\]
Therefore, the likelihood ratio upon not observing $s_{int}$ (i.e. observing $s_{good}$ or $\emptyset$) is at least 
\[
\frac{\mu_{l}(\omega=1)}{\mu_{l}(\omega=0)}\frac{ 1- \frac{\mu_{h}(\omega=0) }{ \mu_{h}(\omega=1)}(b_{1}(\omega=0)\hat{\zeta}(l,d_{min})\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1}) + 2\beta)}{1-  (b_{1}(\omega=0)\hat{\zeta}(l,d_{min})\sum_{s \in S_{int}} \pi_{1}(s|\omega=0)Pr(z \in \hat{L}_{1}) + 2\beta)} 
\]
Then, since the posterior upon observing $s_{good}$ is exactly 0.5, we know that the posterior upon observing $\emptyset$ must also be higher than 0.5. 

Therefore, sender's payoff from $\Pi_{3}^{n}$ is bounded below by
\begin{multline} 
	-\beta v(1)-\beta'+ \sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{3}(\omega) \pi_{3}(s_{good}|\omega)  - 	b_{3}(\omega)\pi_{3}(s_{int}|\omega)v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{3}(\omega) \pi_{3}(s_{good}|\omega)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{3}(\omega)\pi_{3}(s_{int}|\omega)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big]  
\end{multline}
By construction of $\Pi_{3}^{n}$,
\begin{multline}
	\sum_{\omega}\mu_{s}(\omega) b_{3}(\omega)\pi_{3}(s_{int}|\omega)  -\sum_{\omega}\mu_{s}(\omega)b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)  \le \\
	(\mu_{s}(\omega=0)+\mu_{s}(\omega=1)\frac{\mu_{h}(\omega=1) }{\mu_{h}(\omega=0) }  )\frac{4\beta}{(\hat{\zeta}(l,d=1)-2\beta)}   
\end{multline}
Since $b_{1}(\omega)\sum_{s \in S_{good}}\pi_{1}(s|\omega)Pr(z \in L_{1}|s) \le 1-b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)$ , We also know that 
\begin{multline}
	\sum_{\omega}\mu_{s}(\omega)b_{1}(\omega)\sum_{s \in S_{good}}\pi_{1}(s|\omega)Pr(z \in L_{1}|s) -  \sum_{\omega}\mu_{s}(\omega) b_{3}(\omega)\pi_{3}(s_{good}|\omega)  \le \\
	(\mu_{s}(\omega=0)+\mu_{s}(\omega=1)\frac{\mu_{l}(\omega=1) }{\mu_{l}(\omega=0) }  )\frac{4\beta}{(\hat{\zeta}(l,d=1)-2\beta)}  
\end{multline}

Therefore, sender's payoff from $\Pi_{3}^{n}$ is bounded below by
\begin{multline} 
	\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big] \\- \beta v(1)-\beta' -\frac{4\beta}{(\hat{\zeta}(l,d=1)-2\beta)}v(1)(\mu_{s}(\omega=0)+\mu_{s}(\omega=1)\frac{\mu_{l}(\omega=1) }{\mu_{l}(\omega=0) }   + \mu_{s}(\omega=0)+\mu_{s}(\omega=1)\frac{\mu_{h}(\omega=1) }{\mu_{h}(\omega=0) }  )
\end{multline}

Recall that receiver's payoff from $\Pi_{1}$ is bounded above by
\begin{multline} 
	\sum_{\omega}\mu_{s}(\omega) \big[ (1-b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s )  - 	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s))v\big(\sum_{t,d \le \overline{d} }\gamma_{t}p_{d} \alpha(\emptyset,t,d;\Pi^{n}_{1})\big) +\\
	b_{1}(\omega) \sum_{s \in S_{good}} \pi_{1}(s|\omega)Pr(z \in L_{1}|s ) 
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\zeta(t,d) +  p_{d}\gamma_{t}(1-\zeta(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) + \\
	b_{1}(\omega)\sum_{s \in S_{int}}\pi_{1}(s|\omega)Pr(z \in \hat{L}_{1}|s)
	v\big(  \sum_{t,d \le \overline{d} }p_{d}\gamma_{t}
	\hat{\zeta}(t,d) +  p_{d}\gamma_{t}(1-\hat{\zeta}(t,d))\alpha(\emptyset,t,d;\Pi^{n}_{1}) \big) 
	\big]  \beta v(1) + \beta'
\end{multline}
Since $v(1)$ is bounded, and we can choose $\beta$ and $\beta'$ to be arbitrarily small, The result follows. 

